Tiered Reinforcement Learning: Pessimism in the Face of Uncertainty and Constant Regret

We propose a new learning framework that captures the tiered structure of many real-world user-interaction applications, where the users can be divided into two groups based on their different tolerance on exploration risks and should be treated separately. In this setting, we simultaneously maintain two policies $\pi^{\text{O}}$ and $\pi^{\text{E}}$: $\pi^{\text{O}}$ ("O" for "online") interacts with more risk-tolerant users from the first tier and minimizes regret by balancing exploration and exploitation as usual, while $\pi^{\text{E}}$ ("E" for "exploit") exclusively focuses on exploitation for risk-averse users from the second tier utilizing the data collected so far. An important question is whether such a separation yields advantages over the standard online setting (i.e., $\pi^{\text{E}}=\pi^{\text{O}}$) for the risk-averse users. We individually consider the gap-independent vs.~gap-dependent settings. For the former, we prove that the separation is indeed not beneficial from a minimax perspective. For the latter, we show that if choosing Pessimistic Value Iteration as the exploitation algorithm to produce $\pi^{\text{E}}$, we can achieve a constant regret for risk-averse users independent of the number of episodes $K$, which is in sharp contrast to the $\Omega(\log K)$ regret for any online RL algorithms in the same setting, while the regret of $\pi^{\text{O}}$ (almost) maintains its online regret optimality and does not need to compromise for the success of $\pi^{\text{E}}$.

==> LSVI-LCB_and_LSVI-UCB.tex <==

\section{Some Guarantees}
Linear setting as an example. 
\paragraph{Pessimistic LSVI-UCB}
Suppose we run PEVI in \citep{jin2021pessimism} with a given dataset $D$, we have:
\begin{align*}
    V^* - V^{\bpi_k} \leq 2\beta \EE_{\pi^*}[\sum_{h=1}^H \sqrt{\phi(s_h,a_h)\trans\Sigma_h^{-1}\phi(s_h,a_h)}]:=\Delta_{P,k}
\end{align*}
\paragraph{Optimistic LSVI-UCB}
Suppose we run LSVI-UCB in \citep{jin2020provably} with a given dataset $D$, we have:
\begin{align*}
    V^* - V^{\pi_k} \leq 2\beta \EE_{\pi_k}[\sum_{h=1}^H \sqrt{\phi(s_h,a_h)\trans\Sigma_h^{-1}\phi(s_h,a_h)}]:=\Delta_{O,k}
\end{align*}

\paragraph{Informal Comparison between $\Delta_O$ and $\Delta_P$}
The gap between $\Delta_O$ and $\Delta_P$ should be instance-dependent. Intuitively, it depend on how often $Alg^O$ select policies $\pi_k$ which has non-trivial overlaps with $\pi^*$. 

Take the finite-arm bandit problem as an example. If all the arms are BeRegret(0.5) except that the optimal one is BeRegret(0.5+$\epsilon$), then $\Delta_P \approx \Delta_O$. However, as long as we modify one arm from BeRegret(0.5) to Ber (0.4), the difference is clear.

\begin{proposition}[Informal (To check later)]
In the multi-arm bandit problem, suppose we have $\mu_1 \geq \mu_2 \geq...\geq \mu_A$. Denote $\Delta_i = \mu_i - \mu_1.\forall i \geq 2$. We should have:
\begin{align*}
    \sum_{k=1}^K \Delta_{O,k} - \Delta_{P,k} \approx \sum_{i=2}^A \frac{\log K}{2\Delta_i}
\end{align*}
however...
\begin{align*}
    \sum_{k=1}^K \Delta_{O,k} \approx \sum_{i=2}^A \frac{\log K}{\Delta_i}
\end{align*}
which means the improvement is at the constant level...
\end{proposition}

\paragraph{Does there exist other methods to further reduce the regret of $Alg^P$?}

==> arxiv /Behavior_Analysis_of_AlgO.tex <==
\section{Behavior Analysis of Optimistic Algorithm}
\begin{definition}[Definition of Events]\label{def:policy_agreements_events}
\begin{align*}
    &\cE_{k,h,\pi}:=\{\pi_{k,h}(s_h)\neq \pi_{h}(s_h)\},\quad \tilde{\cE}_{k,h,\pi}:=\cE_{k,h,\pi}\cap \bigcap_{\ph=1}^h \cE_{k,\ph-1,\pi}^\complement,\quad \bar{\cE}_{k,\pi}:=\bigcup_{h=1}^H \cE_{k,h,\pi},\\
    &\cE_{k,h}:=\{\pi_{k,h}(s_h)\not\in \Pi^*_{h}(s_h)\},\quad \tilde{\cE}_{k,h,}:=\cE_{k,h}\cap \bigcap_{\ph=1}^h \cE_{k,\ph-1}^\complement,\quad \bar{\cE}_k:=\bigcup_{h=1}^H \cE_{k,h}\\
\end{align*}
\end{definition}
In another word, $\cE_{k,h,\pi}$ means $\pi_k$ disagrees with $\pi$ at state $s_h$ which occurs at step $h$, $\tilde{\cE}_{k,h,\pi}$ means the first disagreement between $\pi_k$ and $\pi$ occurs at step $h$, and $\bar{\cE}_{k,\pi}$ denotes the event that there exists one state $s_h$ at some time step $h\in[H]$ such that $\pi_k$ agrees with $\pi_k$ at $s_h$.

Besides, $\cE_{k,h}$ denotes the events that $\pi_{k,h}(s_h)$ will not be taken by any optimal policy. Note that here we use $\Pi^*_h(s_h)$ to denote the set of all possible optimal actions at state $s_h$. Given a deterministic optimal policy $\pi^*$, in general $\cE_{k,h} \neq \cE_{k,h,\pi^*}$ when there are multiple optimal actions at one state.

\begin{lemma}\label{lem:value_decomposition}
    For arbitrary reward function $R$, given a fixed deterministic policy $\pi$, we have:
    \begin{align*}
        V^{\pi}_1(s_1) - V^{\pi_k}_1(s_1) = &\EE_{\pi_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h,\pi}](V^{\pi}_h(s_h)-V^{\pi_k}_h(s_h))]
    \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        V^{\pi}_1(s_1) - V^{\pi_k}_1(s_1) =& \mathbb{I}[{\cE}_{k,1,\pi}^\complement] \Big(Q^{\pi}_1(s_1,\pi_k)-Q^{\pi_k}_1(s_1,\pi_k)\Big)+\mathbb{I}[{\cE}_{k,1,\pi}] \Big(V^\pi_1(s_1)-V^{\pi_k}_1(s_1)\Big)\\
        =& \EE_{\pi_k}[\mathbb{I}[{\cE}_{k,1,\pi}^\complement]\Big(V^{\pi}_2(s_2)-V^{\pi_k}_2(s_2)\Big)]+\mathbb{I}[\tilde{\cE}_{k,1,\pi}] \Big(V^\pi_1(s_1)-V^{\pi_k}_1(s_1)\Big)\tag{$\tilde{\cE}_{k,1,\pi}=\cE_{k,1,\pi}$ by definition}\\
        =& \EE_{\pi_k}[\mathbb{I}[{\cE}_{k,2,\pi}^\complement\cap {\cE}_{k,1,\pi}^\complement]\Big(Q^{\pi}_2(s_2,\pi_k)-Q^{\pi_k}_2(s_2,\pi_k)\Big)]\\
        &+\EE_{\pi_k}[\mathbb{I}[{\cE}_{k,2,\pi}\cap {\cE}_{k,1,\pi}^\complement]\Big(V^{\pi}_2(s_2)-V^{\pi_k}_2(s_2)\Big)]+\mathbb{I}[\tilde{\cE}_{k,1,\pi}] \Big(V^\pi_1(s_1)-V^{\pi_k}_1(s_1)\Big)\\
        =& \EE_{\pi_k}[\mathbb{I}[{\cE}_{k,2,\pi}^\complement\cap {\cE}_{k,1,\pi}^\complement]\Big(Q^{\pi}_2(s_2,\pi_k)-Q^{\pi_k}_2(s_2,\pi_k)\Big)]\\
        &+\EE_{\pi_k}[\mathbb{I}[\tilde{\cE}_{k,2,\pi}]\Big(V^{\pi}_2(s_2)-V^{\pi_k}_2(s_2)\Big)]+\mathbb{I}[\tilde{\cE}_{k,1,\pi}] \Big(V^\pi_1(s_1)-V^{\pi_k}_1(s_1)\Big)\\
        =&...\\
        =&\EE_{\pi_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h,\pi}](V^{\pi}_h(s_h)-V^{\pi_k}_h(s_h))]
    \end{align*}
\end{proof}
\begin{lemma}[Relationship between Density Difference and Policy Disagreement Probability]\label{lem:relationship_between_occupancy_and_failure_rate}
    \begin{align*}
        d^{\pi_k}(s_h,a_h) \geq d^{\pi}(s_h,a_h) - \min\{\Pr(\bar{\cE}_{k,\pi}|\pi_k),~d^\pi(s_h,a_h)\},\quad \forall s_h\in\cS_h,a_h\in\cA_h,h\in[H]
    \end{align*}
    where we use $\Pr(\bar{\cE}_{k,\pi}|\pi_k)$ as a short note of $\EE_{s_1,a_1,s_2,a_2...,s_H,a_H \sim \pi_k}[\bar{\cE}_{k,\pi}]$.
\end{lemma}
\begin{proof}
    By applying Lemma \ref{lem:value_decomposition} with $\delta_{s_h,a_h}:=\mathbb{I}[S_h=s_h,A_h=a_h]$ as reward function, we have:
    \begin{align*}
        d^{\pi}(s_h,a_h) - d^{\pi_k}(s_h,a_h) = & V^{\pi}_1(s_1;\delta_{s_h,a_h}) - V^{\pi_k}_1(s_1;\delta_{s_h,a_h}) \\
        =&\EE_{\pi_k}[\sum_{\ph=1}^h \mathbb{I}[\tilde{\cE}_{k,\ph,\pi}](V^{\pi}_\ph(s_\ph;\delta_{s_h,a_h})-V^{\pi_k}_\ph(s_\ph;\delta_{s_h,a_h}))] \tag{$V_\ph^\pi = V_\ph^{\pi_k} =0$ for all $\ph \geq h+1$}\\
        \leq& \EE_{\pi_k}[\sum_{\ph=1}^h \mathbb{I}[\tilde{\cE}_{k,\ph,\pi}] V^{\pi}_\ph(s_\ph;\delta_{s_h,a_h})]\tag{$V^{\pi_k}_{h'}(s_h';\delta_{s_h,a_h}) \geq 0$} \\
        \leq& \EE_{\pi_k}[\sum_{\ph=1}^h \mathbb{I}[\tilde{\cE}_{k,\ph,\pi}]] \tag{$V^{\pi}_{h'}(s_h';\delta_{s_h,a_h}) \leq 1$} \\
        \leq& \EE_{s_1,a_1,s_2,a_2...,s_H,a_H \sim \pi_k}[\bar{\cE}_{k,\pi}] = \Pr(\bar{\cE}_{k,\pi}|\pi_k)
    \end{align*}
    which implies that,
    \begin{align*}
        d^{\pi_k}(s_h,a_h) \geq d^{\pi}(s_h,a_h) - \Pr(\bar{\cE}_{k,\pi}|\pi_k)
    \end{align*}
    Combining with $d^{\pi_k} \geq 0$, we finish the proof.
\end{proof}

\begin{definition}[Conversion to Optimal Deterministic Policy]\label{def:conversion_to_opt_det_policy}
    Given arbitrary deterministic policy $\pi=\{\pi_1,...,\pi_H\}$, we use $\Pi^*\circ \pi=\{\pi_1^*,...,\pi^*_H\}$ to denote an optimal deterministic policy, such that:
    \begin{align*}
        \pi^*_{h}(s_h) = \begin{cases}
            \pi_{h}(s_h),\quad & \text{if}~\pi_{h}(s_h)\in \Pi^*_h(s_h);\\
            \text{Select}(\Pi^*_h(s_h)),\quad &\text{otherwise}.
        \end{cases}
    \end{align*}
    where $\text{Select}$ is a function which returns the first optimal action from $\Pi^*_h(s_h)$.
\end{definition}
In another word, $\Pi^*\circ\pi$ agrees with $\pi$ if $\pi_{h}(s_h)$ is one of the optimal action at state $s_h$. Otherwise, $\Pi^*\circ\pi$ takes one of a fixed optimal action from $\Pi^*_h(s_h)$. In order to make sure $\Pi^*\circ$ is a deterministic mapping, we assume function $Select$ only choose the first optimal action in $\Pi^*(s_h)$ (ordered by index of action).

\ThmORegretPDensity*
\begin{proof}
    For each $\pi_k$, we construct an optimal deterministic policy $\pi^*_k:=\Pi^*\circ\pi_k$, where $\Pi^*\circ$ is defined in Def. \ref{def:conversion_to_opt_det_policy}.
    By applying Lemma \ref{lem:value_decomposition} with the reward function in MDP, and $\pi=\pi_k^*$, we have:
    \begin{align*}
        V^{\pi^*_k}_1(s_1) - V^{\pi_k}_1(s_1) = &\EE_{\pi_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h,\pi_k^*}](V^{\pi^*_k}_h(s_h)-V^{\pi_k}_h(s_h))] \\
        \geq& \EE_{\pi_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h,\pi_k^*}](V^{\pi^*_k}_h(s_h)-Q^{\pi^*_k}_h(s_h, \pi_k(s_h)))]\\
        \geq& \EE_{\pi_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h,\pi_k^*}]\Delta_{\min}]=\Delta_{\min} \Pr(\bar{\cE}_{k,\pi_k^*}|\pi_k)
        % =\Delta_{\min} \Pr(\bar{\cE}_{k}|\pi_k)
    \end{align*}
    % where the last step is because of the way we construct $\pi_k^*$.
    Therefore, we have:
    \begin{align*}
        \Pr(\bar{\cE}_{k,\pi_k^*}|\pi_k) \leq \frac{1}{\Delta_{\min}}(V^{\pi^*_k}_1(s_1)-V^{\pi_k}_1(s_1))
    \end{align*}
    % Because of the above construction, that $\pi_k(s_h)$ is not one of optimal actions if and only if $\pi_k\neq \pi_k^*$, which implies that:
    % \begin{align*}
    %     \cE_{k,h,\pi^*}=\cE_{k,h}
    % \end{align*}
    % and therefore,
    % \begin{align*}
    %     \Pr(\bar{\cE}_{k,\pi_k^*}^\complement|\pi_k)=\Pr(\bar{\cE}_{k}^\complement|\pi_k)\leq \frac{1}{\Delta_{\min}} \Big(V^*_1(s_1)-V^{\pi_k}_1(s_1)\Big)
    % \end{align*}
    By applying Lemma \ref{lem:relationship_between_occupancy_and_failure_rate}, we have:
    \begin{align*}
        d^{\pi_k}(s_h,a_h) \geq d^{\pi_k^*}(s_h,a_h) - \frac{1}{\Delta_{\min}} \Big(V^*_1(s_1)-V^{\pi_k}_1(s_1)\Big),\quad\forall s_h\in\cS_h,a_h\in\cA_h,h\in[H]
    \end{align*}
    After the same discussion for all $k\in[K]$, and the above inequality of each $k$ together, we have:
    \begin{align*}
        \sum_{k=1}^K d^{\pi_k}(s_h,a_h) \geq \sum_{k=1}^K d^{\pi^*_k}(s_h,a_h) - \frac{1}{\Delta_{\min}} (\sum_{k=1}^K V^*_1(s_1)-V^{\pi_k}_1(s_1)\Big)
    \end{align*}
\end{proof}

% \paragraph{Some addtional notations}
% Moreover, we use $\Pi^*_h(s_h)$ to denote all the optimal actions at state $s_h$ and use $|\Pi^*_h(s_h)|$ to denote its cardinality. As extensions, we define $|\Pi^*_h(\cS^*_h)|:=\sum_{s_h\in\cS^*_h}|\Pi^*_h(s_h)|$, $|\Pi^*_h(\cS^*_{h,\text{div}})|:=\sum_{s_h\in\cS^*_{h,\text{div}}}|\Pi^*_h(s_h)|$. 
% Note that: $\cZ_{h,\text{div}}^* \subset \cZ_{h}^* \subset \cZ_{h}$, and therefore, 
% $$
% |\cZ_{h,\text{div}}^*| \leq |\cZ_{h}^*| \leq |\cZ_{h}| = SA
% $$
% Moreover, when there is only one optimal deterministic policy, we have $|\cZ_{h,\text{div}}^*| =0$.
% $$
% |\Pi^*_h(\cS^*_{h,\text{div}})| \leq |\Pi^*_h(\cS^*_h)| \leq |\cS^*_h| \cdot \max_{s_h\in\cS^*_h}|\Pi^*_h(s_h)| \leq SA
% $$


\begin{corollary}[Unique Optimal Policy]\label{corl:unique_optimal_policy}
    When $|\Pi^*|=1$, Thm. \ref{thm:algO_regret_vs_algP_density} implies that:
    \begin{align*}
        \sum_{k=1}^K d^{\pi_k}(s_h,a_h) \geq K d^{\pi^*}(s_h,a_h) - \frac{1}{\Delta_{\min}} (\sum_{k=1}^K V^*_1(s_1)-V^{\pi_k}_1(s_1)\Big)
    \end{align*}
\end{corollary}

\ThmExistWellCovered*
\begin{proof}
    For arbitrary $h\in [H]$, we define: 
    \begin{align*}
        N_{I_K^*}(s_h,a_h):=\sum_{k=1}^K \mathbb{I}[d^{\pi^*_k}(s_h,a_h) > 0]
    \end{align*}
    In another word, $N_{I_K^*}(\cdot,\cdot)$ denotes the number of optimal policies in the sequence, which can hit state $s_h$ and take action $a_h$. 
    % Obviously, for each $h\in[H]$, there are at most $|\Pi^*_h(\cS^*_h)| \leq SA$ state action pairs with positive value of $N_{I_K^*}$.
    
    Next, we define $\cZ_h^*$, $\cZ_{h}^{\text{insuff}}$ and $\Pi_{h,\text{insuff}}$ as
    \begin{align*}
        \cZ_h^*:=&\{(s_h,a_h)\in\cS_h,\cA_h|\exists \pi^*\in\Pi^*,~s.t.~d^{\pi^*}(s_h,a_h) > 0\}\\
        \cZ_{h}^{\text{insuff}}:= &\{(s_h,a_h)|(s_h,a_h)\in\cZ^*_h:~N_{I_K^*}(s_h,a_h)<\frac{K}{2(|\cZ^*_{h,\text{div}}|+1)H}\}\\
        I_h^{\text{insuff}}:= &\{k\in[K]:~\exists (s_h,a_h)\in\cZ_{h}^{\text{insuff}},~s.t.~d^{\pi_k}(s_h,a_h) > 0\}
    \end{align*}
    In a word, $\cZ_h^*$ is the collection of states actions reachable by at least one optimal policy, $\cZ_{h}^{\text{insuff}}$ is a collection of ``insufficiently hitted'' states actions at step $h$, which are only covered by a small portion of optimal policies in the sequence, and $I_h^{\text{insuff}}$ is a collection of the index of the optimal policies in the sequence, which cover at least one state action pair in $\cZ_{h}^{\text{insuff}}$. 

    % Besides, we use $\bar{s}_h,\bar{a}_h$ to denote the state action pair which maximizes $N_{I_K^*}(\cdot,\cdot)$, and because the maximum is always no less than the average, we have:
    % \begin{align*}
    %     N_{I_K^*}(\bar{s}_h,\bar{a}_h) \geq \frac{1}{2|\Pi^*_h(\cS^*_h)|}\sum_{s_h\in\cS_h}\sum_{a_h\in\Pi^*_h(s_h)}N_{I_K^*}(s_h,a_h) \geq \frac{K}{2|\Pi^*_h(\cS^*_h)|}
    % \end{align*}
    % Easy to see that $(\bar{s}_h,\bar{a}_h) \not\in\cZ_{h}^{\text{insuff}}$. 
    
    Note that we must have $\cZ_{h}^{\text{insuff}}\subset \cZ_{h,\text{div}})$, because if one state action pair $s_h,a_h$ is reachable by arbitrary deterministic policy, then $N_{I^*_k}(s_h,a_h) = K$. Then, we have:
    \begin{align*}
        |I_h^{\text{insuff}}| < |\cZ_{h}^{\text{insuff}}|\cdot \frac{K}{2(|\cZ_{h,\text{div}}|+1) H} \leq |\cZ_{h,\text{div}}|\cdot \frac{K}{2(|\cZ_{h,\text{div}}|+1) H} \leq \frac{K}{2H}
    \end{align*}
    We define $I_{1:H}^{\text{suff}}:=I_K \setminus \bigcup_{h=1}^H I_h^{\text{insuff}}$. Intuitively, $I_{1:H}^{\text{suff}}$ is the set including the indices of optimal policies in the sequence only hitting those states which are covered by most of the other optimal policies. In fact, $I_{1:H}^{\text{suff}}$ is non-empty since:
    \begin{align*}
         |I_{1:H}^{\text{suff}}|\geq K - \frac{K}{2H} \cdot H = \frac{K}{2}
    \end{align*}
    We use $\pi^*_{I_{1:H}^{\text{suff}}}$ to denote the average mixture policy over $\{\pi_i^*: i\in I_{1:H}^{\text{suff}}\}$, a direct result is that:
    \begin{align*}
        \sum_{k=1}^K d^{\pi^*_k}(s_h,a_h) \geq \sum_{k\in I_{1:H}^{\text{suff}}} d^{\pi^*_k}(s_h,a_h) = |I_{1:H}^{\text{suff}}|\cdot d^{\pi^*_{I_{1:H}^{\text{suff}}}} \geq \frac{K}{2}\cdot d^{\pi^*_{I_{1:H}^{\text{suff}}}}
    \end{align*}
    On the other hand, for all $s_h,a_h$ such that $d^{\pi^*_{I_{1:H}^{\text{suff}}}}(s_h,a_h) > 0$, we must have $(s_h,a_h)\not\in \cZ_{h}^{\text{insuff}}$, and therefore:
    \begin{align*}
        \sum_{k=1}^K d^{\pi^*_k}(s_h,a_h) \geq \frac{K}{2(|\cZ_{h,\text{div}}|+1)H}d^*_{h,\min}(s_h,a_h)
    \end{align*}
    Combining the above two inequalities, we finish the proof.
\end{proof}









\iffalse 
Recall that given arbitrary policy $\pi_k$, the value gap can be represented by:
\begin{align*}
    V^* - V^{\pi_k} = \EE_{\pi_k}[\sum_{h=1}^H \Delta_h(s_h,a_h)]
\end{align*}
Note that:
\begin{align*}
    \text{Regret}(Alg^O) = \sum_{k=1}^K V^* - V^{\pi_k} = \sum_{k=1}^K \EE_{\pi_k}[\sum_{h=1}^H \Delta_h(s_h,a_h)]
\end{align*}

We use $\{s_{k,h},a_{k,h}\}_{h=1}^H$ to denote the trajectory sampled by executing $\pi_k$ after computing $\pi_k$ at iteration $k$. Note that $Z_k = V^* - V^{\pi_k} - \sum_{h=1}^H \Delta_h(s_{k,h},a_{k,h})=\EE_{\pi_k}[\sum_{h=1}^H \Delta_h(s_h,a_h)]-\sum_{h=1}^H \Delta_h(s_{k,h},a_{k,h})$ is a martingale difference sequence with expectation zero and
\begin{align*}
    |Z_k| =& |\EE_{\pi_k}[\sum_{h=1}^H \Delta_h(s_h,a_h)]-\sum_{h=1}^H \Delta_h(s_{k,h},a_{k,h})| \leq \max\{|V^* - V^{\pi_k}|, \sum_{h=1}^H\max_{s_h,a_h}|\Delta_h(s_h,a_h)|\}\\
    \leq &\max\{H, \sum_{h=1}^H (H-h)\} \leq H^2
\end{align*}
Then we have, with probability $1-\delta$,
\begin{align*}
    \sum_{k=1}^K Z_k \geq -H^2\sqrt{2K\log \frac{1}{\delta}}
\end{align*}
which implies that,
\begin{align*}
    \sum_{k=1}^K \sum_{h=1}^H \Delta_h(s_{k,h},a_{k,h}) \leq H^2\sqrt{2K\log \frac{1}{\delta}} + \sum_{k=1}^K V^* - V^{\pi_k}
\end{align*}
We use $N_{k,h}$ to denote the sequence $\{(s_{k,h},a_{k,h})\}_{h=1}^H$ such that $\Delta_h(s_h,a_h)=0$ for all $h\in [H]$ up to iteration $k$, we should have:
\begin{align*}
    \sum_{k=1}^K \sum_{h=1}^H \Delta_h(s_{k,h},a_{k,h}) \geq (K-N_{k,h}) \Delta_{\min}
\end{align*}
Therefore,
\begin{align*}
    N_{k,h} \geq K - \frac{H^2\sqrt{2K\log \frac{1}{\delta}} + \sum_{k=1}^K V^* - V^{\pi_k}}{\Delta_{\min}}
\end{align*}

If we have an anytime algorithm, such that for arbitrary $k > 0$, with probability $1-\delta$, we have:
\begin{align*}
    \sum_{k=1}^K V^* - V^{\pi_k} = C_1 + C_2 \log \frac{C_3 K}{\delta}
\end{align*}
For arbitrary $k > 0$, we choose $\delta = 1/k^{\alpha}$, such that with probability $1 - 2/k^\alpha$, we have:
\begin{align*}
    N_{k,h} \geq K - \frac{H^2 \sqrt{2\alpha K \log K}+C_1+C_2 \alpha \log C_3 K}{\Delta_{\min}}
\end{align*}
which implies that, after a few time steps, we have $N_{k,h} \geq K$.
\fi


==> arxiv /Experiments.tex <==
\section{Experiments}\label{appx:experiments}
% We provide some simulation results in tabular MDP in this section.
\subsection{Experiment Setup}
\paragraph{Environment}
We test our algorithms in tabular MDPs with randomly generated transition and rewards functions. To generate the MDP, for each layer $h$ and each state action pair $(s_h,a_h)$, we first sample a random vector $\mP(\cdot|s_h,a_h)$, where each element is uniformly sampled from $\{1,2,3...,10\}$, and then normalize it to a valid probability vector. Besides, the reward function is set to $\xi/10$ where $\xi$ is randomly generated from $\{1,2,...,10\}$ to make sure it locates in $[0,1]$.

\paragraph{Algorithm}
We implement the StrongEuler algorithm in \citep{simchowitz2019non} as $\algO$ and construct the same adaptive bonus term (Alg. 3 in \citep{simchowitz2019non}) for $\algE$ to match Cond. \ref{cond:bonus_term}.
Although for the convenience of analysis, in our Framework \ref{alg:general_learning_framework}, we do not consider to use the data generated by $\algE$, in experiments, we use both $\tauO$ and $\tauE$, which slightly improves the performance.
Besides, in practice, we observe that the bonus term is quite loose, and it will take a long time before the estimated $Q/V$ value fallen in the interval $[0, H]$, which is the value range of true value functions.
Therefore, we introduce a multiplicator $\alpha$ and adjust the bonus term from $b_{k,h}$ to $\alpha \cdot b_{k,h}$, and set $\alpha = 0.25$ for both $\algO$ and $\algE$.

\subsection{Results}
We test the algorithms in tabular MDPs with $S=A=H=5$\footnote{The code can be find in \url{https://github.com/jiaweihhuang/Tiered-RL-Experiments}.}. Although the minimal gap $\Delta_{\min}$ is hard to control since we generate the MDP in a random way, we filter out three random seeds in MDP construction, which correspond to minimal gaps (approximately) equal to 0.0015, 0.003 and 0.009, respectively. We report the accumulative regret in Fig. \ref{fig:simulation_results}.

As predicted by our theory, $\algE$ can indeed achieve constant regret in contrast with the continuously increasing regret of $\algO$, which demonstrates the advantage of leveraging tiered structure.
\begin{figure}
    \centering
    % \subfigure[$\Delta_{\min}\approx 0.0015$]{
    %     \includegraphics[scale=0.2]{Pictures/S5-A5-H5-GapMin0.001.png}
    %     % \caption{$\Delta_{\min}\approx 0.001$}
    % }
    % \subfigure[$\Delta_{\min}\approx 0.003$]{
    % \includegraphics[scale=0.2]{Pictures/S5-A5-H5-GapMin0.003.png}
    % }
    % \subfigure[$\Delta_{\min}\approx 0.009$]{
    % \includegraphics[scale=0.2]{Pictures/S5-A5-H5-GapMin0.009.png}
    % }
    \includegraphics[scale=0.45]{Pictures/Results.png}
    \caption{Simulation results with $S=A=H=5$ and different $\Delta_{\min}$, averaged over 10 different random seeds. Error bars show double the standard errors, which correspond to 95\% confidence intervals. Our choice of $\algE$ can achieve constant regret as predicted by theory. We can also see the tendency that larger $\Delta_{\min}$ will result in smaller accumulative regret.}
    \label{fig:simulation_results}
\end{figure}

==> arxiv /Extension_on_Tabular_MDP_Regret.tex <==
\section{Analysis of Pessimistic Value Iteration}\label{appx:analysis_of_PVI}

In this section, we provide analysis for Alg. \ref{alg:PVI}. Our analyses base on an extension of the Clipping Trick in \citep{simchowitz2019non} into our setting. 
% In this section, we mainly focus on how to use some intermediate level lemma to provide an upper bound for the regret of $\algE$, and defer the detailed discussion about the extended clipping trick and related lemma and their proofs to Appx. \ref{appx:clipTrick_and_Surplus}.

\subsection{Underestimation and Some Concrete Choices of Bonus Term}\label{appx:choice_of_bonus_term}
\begin{lemma}[Underestimation]\label{lem:underest_PVI}
    Given a $\textbf{Bonus}$ satisfying Cond. \ref{cond:bonus_term}, for arbitrary dataset $D_k$ consisting of $k$ trajectories by a sequence of policies $\pi_1,...,\pi_k$, by running Alg \ref{alg:PVI} with $D_k$ and the bonus term $b(\cdot,\cdot)$ returned by $\textbf{Bonus}(D_k,\delta_k)$, on the events $\cEB$ defined in Cond. \ref{cond:bonus_term}:
    \begin{align}
        \forall h\in[H],\forall s_h\in\cS_h,a_h\in\cA_h,\quad \hQ_h(s_h,a_h) \leq Q^{\pi_{\hQ,h}}(s_h,a_h) \leq Q^{*}(s_h,a_h) \label{eq:under_estimation}
    \end{align}
    where we use $\pi_\hQ=\{\pi_{\hQ,1},...,\pi_{\hQ,H}\}$ to denote the greedy policy w.r.t. $\hQ$.
\end{lemma}
\begin{proof}
    We only prove the first inequality holds, since the second one holds directly because of the definition of optimal policy.

    First of all, $V_{H+1} = 0 \leq V^{\pi_\hQ}_{H+1}$ holds directly, which implies that Eq.\eqref{eq:under_estimation} holds at step $h=H$ as a result of the deterministic reward function. 
    
    Now, we conduct the induction. Suppose Eq.\eqref{eq:under_estimation} already holds for $h+1$, which implies that:
    \begin{align}
        \hV_{h+1}(s_{h+1}) = \hQ_{h+1}(s_{h+1},\pi_{\hQ, h+1}(s_{h+1})) \leq Q^{\pi_\hQ}_{h+1}(s_{h+1},\pi_{\hQ, h+1}(s_{h+1})) = V^{\pi_\hQ}_{h+1}(s_{h+1})\label{eq:under_est_mid_step}
    \end{align}
    then, at step $h$, we have:
    \begin{align*}
        Q_h(s_h,a_h) - Q^{\pi_\hQ}(s_h,a_h) =& \hat P_h \hV_{h+1} (s_h,a_h) - b_h(s_h,a_h) - P_hV^\pi_{h+1}(s_h,a_h)\\
        =& \underbrace{(\hat P_h - P_h)\hV_{h+1}(s_h,a_h) - b_h(s_h,a_h)}_{\text{part 1}} + \underbrace{P_h(\hV_{h+1}-V_{h+1}^{\pi_\hQ})(s_h,a_h)}_{\text{part 2}}
    \end{align*}
    As we can see, part 1 is non-positive with probability $1-\delta$ as a result of Cond. \ref{cond:bonus_term}, while part 2 is also less than or equal to zero because of the induction condition in Eq.\eqref{eq:under_est_mid_step}.
\end{proof}

\paragraph{Choice 1: Naive Bound}
According to Hoeffding inequality, with probability $1-\delta/(SAH)$, we have the following holds for each $s_h,a_h,h$
\begin{align*}
    |\hP_h V_{h+1} - P_h V_{h+1}| \leq \|\hP_h - P_h\|_1 \|V_{h+1}\|_\infty \leq \|\hP_h - P_h\|_1H \leq c_1 HS \sqrt{\frac{\log(SAH/\delta)}{N(s_h,a_h)}}
\end{align*}
which implies that condition \ref{cond:bonus_term} holds with probability $1-\delta$ as long as:
\begin{align*}
    b_h(N, \delta) := HS \sqrt{\frac{\log(SAH/\delta)}{N}}
\end{align*}

\paragraph{Choice 2: Adaptive Bonus Term based on the ``Bernstein Trick''}
One can also consider an analogue of the bonus term functions in Alg. 3 of \citep{simchowitz2019non}, which is originally designed for optimistic algorithms. We omit the discussions here.

\input{Appendix/Appx_ClippingTrick}

\subsection{Upper Bound for the Regret of $\algE$}
\ThmClipTrick*
\begin{proof}
    We separately discuss the cases when there are unique or multiple deterministic optimal policies.
    \paragraph{Case 1: Unique Deterministic Optimal Policy}
    % Recall the definition of $\ddot{V}^{\pi^*}$ in Appx. \ref{appx:clipTrick_and_Surplus}. 
    For arbitrary $h,s_h$, suppose $\piPVI_k(s_h)\not\in\Pi^*(s_h)$, we have:
    \begin{align*}
        V^*_h(s_h) - \ddot{V}^{\pi^*}_{k,h}(s_h) \geq& V_h^*(s_h) - \hV_{k,h}(s_h) - (H-h+1)\epsClip \\
        \geq & \frac{1}{2}\Big(V_h^*(s_h) - \hV_{k,h}(s_h)\Big) + \frac{1}{2}\Big(V_h^*(s_h) - V_h^{\piPVI_k}(s_h)\Big) - \frac{\Delta_{\min}}{2}\\
        \geq & \frac{1}{2}\Big(V_h^*(s_h) - \hV_{k,h}(s_h)\Big) + \frac{1}{2}\Big(V_h^*(s_h) - Q_h^*(s_h,\piPVI_k)\Big) - \frac{\Delta_{\min}}{2}\\
        = & \frac{1}{2}\Big(V_h^*(s_h) - \hV_{k,h}(s_h)\Big) + \frac{\Delta_h(s_h,\piPVI_k(s_h))}{2} - \frac{\Delta_{\min}}{2} \\
        \geq& \frac{1}{2}\Big(V_h^*(s_h) - \hV_{k,h}(s_h)\Big)
        % \geq& \frac{1}{2}\Big(V_h^*(s_h) - \hQ_{k,h}(s_h,a_h^*)\Big),\quad \forall a_h^* \in \Pi^*(s_h)
    \end{align*}
    Recall the definition of Events in Def.\ref{def:policy_agreements_events}, and note that when the optimal policy is unique, the events $\tilde{\cE}_{k,h,\pi^*}, \bar{\cE}_{k,h,\pi^*}$ collapse to $\tilde{\cE}_{k,h}, \bar{\cE}_{k,h}$, respectively. For arbitrary optimal policy $\pi^*$, we have:
    \begin{align*}
        V^*_1(s_1) - \ddot{V}^{\pi^*}_1(s_1) =& V^{\pi^*}_1(s_1) - \ddot{V}^{\pi^*}_1(s_1)\\
        =& \mathbb{I}[\cE_{k,1}]\Big(V^*_1(s_1) - \ddot{V}_{1}^{\pi^*}(s_1)\Big) + \mathbb{I}[\cE_{k,1}^\complement]\Big(V^*_1(s_1) - \ddot{V}_{1}^{\pi^*}(s_1)\Big)\\
        \geq& \mathbb{I}[\cE_{k,1}]\frac{1}{2}\Big(V^*_1(s_1) - \hV_{k,1}(s_1)\Big)+ \mathbb{I}[\cE_{k,1}^\complement]\mP (V^*_{2}-\ddot{V}_{2}^{\pi^*})(s_1,\pi^*)\\
        \geq& ...\\
        \geq&\frac{1}{2} \EE_{\pi^*}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h}] (V_h^*(s_h) - \hV_{k,h}(s_h))]
    \end{align*}
    Besides, on the other hand,
    \begin{align*}
        V_1^*(s_1)-V^{\piPVI_k}_1(s_1) 
        =& \mathbb{I}[\cE_{k,1}](V_1^{\pi^*} - V^{\piPVI_k}_1(s_1)) + \mathbb{I}[\cE_{k,1}^\complement](V_1^{\pi^*} - Q^{\piPVI_k}_1(s_1,\pi^*)) \\
        =& \mathbb{I}[\cE_{k,1}](V_1^{\pi^*} - V^{\piPVI_k}_1(s_1)) + \mathbb{I}[\cE_{k,1}^\complement]\mP_1(V_2^* - V^{\piPVI_k}_2)(s_1,\pi^*)) \\
        =& ... \\
        =& \EE_{\piPVI_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h}] (V_h^{\pi^*}(s_h) - V^{\piPVI_k}_h(s_h))]\\
        \leq & \EE_{\piPVI_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h}] (V_h^{\pi^*}(s_h) - \hV_{k,h}(s_h))]
    \end{align*}
    Combining the above two results and Lemma \ref{lem:upper_bound_surplus}, we finish the discussion for Case 1.

    % \begin{align*}
    %     V_1^*(s_1)-V^{\piPVI_k}_1(s_1) \leq & V_1^{\pi^*}(s_1)-\hV_{k,1}(s_1)\\
    %     =&\mathbb{I}[\cE_{k,1}](V_1^{\pi^*} - \hV_{k,1}(s_1)) + \mathbb{I}[\cE_{k,1}^\complement](V_1^{\pi^*} - \hV_{k,1}(s_1)) \\
    %     \leq&\mathbb{I}[\cE_{k,1}](V_1^{\pi^*} - \hV_{k,1}(s_1)) + \mathbb{I}[\cE_{k,1}^\complement](V_1^{\pi^*} - \hQ_{k,1}(s_1,\pi^*)) \tag{$\piPVI_k$ is greedy policy} \\
    %     \leq&\mathbb{I}[\cE_{k,1}](V_1^{\pi^*} - \hV_{k,1}(s_1)) + \mathbb{I}[\cE_{k,1}^\complement](\mP_1V_2^{\pi^*}(s_1,\pi^*) - \hmP_1\hV_{k,2}(s_1,\pi^*)) \\
    %     =& \mathbb{I}[\cE_{k,1}](V_1^{\pi^*} - Q^{\pi_k}_1(s_1,\pi_k)) + \mathbb{I}[\cE_{k,1}^\complement](V_1^{\pi^*} - Q^{\pi_k}_1(s_1,\pi^*)) \\
    %     =& \mathbb{I}[\cE_{k,1}](V_1^{\pi^*} - Q^{\pi_k}_1(s_1,\pi_k)) + \mathbb{I}[\cE_{k,1}^\complement]\mP_1(V_2^* - V^{\pi_k}_2)(s_1,\pi^*)) \\
    %     =& ... \\
    %     =& \EE_{\piPVI_k}[\sum_{h=1}^H \mathbb{I}[\tilde{\cE}_{k,h,\pi^*}] (V_1^{\pi^*}(s_h) - V^{\piPVI_k}_h(s_h))]
    % \end{align*}
    
    \paragraph{Case 2: Non-unique Optimal Deterministic Policies}
    From Lemma \ref{lem:relationship_between_value_diff_and_deficit}, we know that,
    \begin{align*}
        V^*_1(s_1) - V^{\piPVI_k}_1(s_1) \leq V^*_1(s_1) - \hV_{k,1}(s_1) \leq& \EE_{\pi^*}[\sum_{h=1}^H \surplus_{k,h}(s_h,a_h)]
    \end{align*}
    where $\pi^*$ can be arbitrary optimal policy. Combining with Lemma \ref{lem:minimal_gap_for_det_subopt_policy}, we know that:
    \begin{align*}
        V^*_1(s_1) - V^{\piPVI_k}_1(s_1) \leq& \Clip[\EE_{\pi^*}[\sum_{h=1}^H \surplus_{k,h}(s_h,a_h)]|d_{\min}\Delta_{\min}]\\
        \leq& 2\sum_{h=1}^H \sum_{s_h\in\cS_h,a_h\in\cA_h} \Clip[d^{\pi^*}(s_h,a_h)\surplus_{k,h}(s_h,a_h)|\frac{d_{\min}\Delta_{\min}}{2SAH}] \tag{Lemma \ref{lem:property_of_clip_operator}}\\
        \leq& 2\sum_{h=1}^H \EE_{\pi^*}[\Clip[\surplus_{k,h}(s_h,a_h)|\frac{d_{\min}\Delta_{\min}}{2SAH}]]
    \end{align*}
    where the last inequality is because $\Clip[\alpha x| \epsilon] < \alpha \Clip[x|\epsilon]$ as long as $\alpha < 1$. Combining with Lemma \ref{lem:upper_bound_surplus}, we finish the proof.
\end{proof}
Next, we introduce a useful Lemma from \citep{dann2017unifying}:
\begin{lemma}[Lemma 7.4 in \citep{dann2017unifying}]\label{lem:concentration}
    Let $\mathcal{F}_i$ for $i,1...$ be a filtration and $X_1,...X_n$ be a sequence of Bernoulli random variables with $\Pr(X_i=1|\mathcal{F}_{i-1})=P_i$ with $P_i$ being $\mathcal{F}_{i-1}$-measurable and $X_i$ being $\mathcal{F}_i$ measurable. It holds that
    \begin{align*}
        \Pr(\exists n: \sum_{i=1}^n X_i < \sum_{i=1}^n P_i / 2 - W) \leq e^{-W}
    \end{align*}
\end{lemma}

\paragraph{Definition of Good Events}
We first introduce some notations about good events which holds with high probability. 
We override the definition in Cond. \ref{cond:bonus_term} by assigning $\delta=\delta_k = 1/k^\alpha$ at iteration $k$, i.e.:
\begin{align*}
    \cEBk :=& \bigcap_{h\in[H],s_h\in\cS_h,a_h\in\cA_h}\Big\{|\hat P_{k,h}V_{k,h+1}(s_h,a_h) - P_hV_{k,h+1}(s_h,a_h)| < b_{k,h}(s_h,a_h)\} \\
    &\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \cap \{b_{k,h}(s_h,a_h) \leq B_1\sqrt{\frac{\log (B_2\cdot k^\alpha)}{N_{k,h}(s_h,a_h)}}\Big\}, \\
    \text{with} &\quad b_k=\{b_{k,1},...,b_{k,H}\} \gets \textbf{Bonus}(D_k,1/k^\alpha).
\end{align*}
Besides, we use $\cECk$ to denote the concentration event that 
\begin{align*}
    \cECk:= \bigcap_{h\in[H],s_h\in\cS_h,a_h\in\cA_h} \{N_{k,h}(s_h,a_h) \geq \frac{1}{2}\sum_{\pk=1}^k d^{\piO_\pk}(s_h,a_h) - \alpha \log(SAHk)\}
\end{align*}
Finally, we use $\cEOk$ to denote the good events that the regret of $\algO$ is only at the level $\log k$:
\begin{align*}
    \cEOk := \{\sum_{\tk=1}^\nk V^*_1(s_1)-V^{\piO_\tk}_1(s_1) < C_1 + \alpha C_2 \log \nk\} 
\end{align*}
Based on Cond. \ref{cond:bonus_term}, Cond. \ref{cond:requirement_on_algO} and Lemma \ref{lem:concentration}, we have:
\begin{align*}
    &\Pr(\cEOk) \geq 1-\frac{1}{k^\alpha}, \quad \Pr(\cEBk) \geq 1 - \frac{1}{k^\alpha}\\
    &\Pr(\cECk) \geq 1 - SAH \cdot \exp(-\alpha \log(SAHk)) = 1 - \frac{SAH}{(SAHk)^\alpha} \geq 1-\frac{1}{k^\alpha}
\end{align*}

\begin{restatable}{lemma}{ThmSubOpt}[One Step Sub-optimality Gap Conditioning on Good Events]\label{thm:SubOpt_under_GoodEvents}
    At iteration $k$, on the good events $\cEBk,\cECk$ and $\cEOk$, the sub-optimality gap of $\piE_k$ can be upper bounded by:
    
    (i) when $|\Pi^*|=1$ (i.e. the optimal deterministic policy is unique):
    \begin{align*}
        V_1^*(s_1) - V^{\piE_k}(s_1) \leq 2\EE_{\pi^*}\Big[\sum_{h=1}^H\Clip\Big[\mathbb{I}[k < \btau^{\pi^*}_{s_h,a_h}]\}\cdot H + \mathbb{I}[k \geq \btau^{\pi^*}_{s_h,a_h}]\cdot B_1\sqrt{\frac{8\alpha \log (B_2 k)}{kd^{\pi^*}(s_h,a_h)}}\Big|\epsClip\Big]\Big]
    \end{align*}

    \indent (ii) when $|\Pi^*|>1$ (i.e. there are multiple optimal deterministic policy):
    \begin{align*}
        V_1^*(s_1) - V^{\piE_k}(s_1) \leq 2\EE_{\pi^*_{\text{cover}}}\Big[\sum_{h=1}^H\Clip\Big[\mathbb{I}[k < \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}]\}\cdot H + \mathbb{I}[k \geq \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}]\cdot B_1\sqrt{\frac{4\alpha \log (B_2 k)}{k\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)}}\Big|\epsClip'\Big]\Big]
    \end{align*}
    where $\epsClip:=\frac{\Delta_{\min}}{2H+2}$ and $\epsClip':=\frac{d_{\min}\Delta_{\min}}{2SAH}$; $\pi^*_{\text{cover}}$ and $\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)$ are defined in Thm. \ref{thm:existence_of_well_covered_optpi}; besides,
    \begin{align*}
        \btau^\pi_{s_h,a_h}:=c_\tau\frac{\alpha(C_1+C_2)}{d^{\pi}(s_h,a_h)\Delta_{\min}} \log \frac{\alpha SAH(C_1+C_2)}{d^{\pi}(s_h,a_h) \Delta_{\min}},\quad \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}:=c'_\tau\frac{\alpha(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)\Delta_{\min}} \log \frac{\alpha SAH(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h) \Delta_{\min}}.
    \end{align*}
    for some constant $c_\tau$, $c'_\tau$.
\end{restatable}
\begin{proof}
% In the following, we provide analysis for the sub-optimality gap for each $\piE_k$ conditioning on the good events $\cEBk, \cECk$ and $\cEOk$ holds.
We first discuss the case when $|\Pi^*|=1$.
\paragraph{Case 1: unique optimal deterministic policy}
As a result of Thm. \ref{thm:clipping_trick}, on the event $\cEBk$, we show that the sub-optimality gap of $\piE_k$ can be upper bounded by:
\begin{align*}
    V^*_1(s_1) - V_1^{\piE_k}(s_1)\leq& 2\EE_{\pi^*}[\sum_{h=1}^H \ddot{\surplus}_{\nk,h}(s_h,a_h)]=\sum_{h=1}^H \sum_{s_h,a_h}d^{\pi^*}(s_h,a_h) \ddot{\surplus}_{\nk,h}(s_h,a_h)
\end{align*}
Because of Lemma \ref{lem:upper_bound_surplus}, the above further implies that:
\begin{align*}
    V^*_1(s_1) - V_1^{\piE_k}(s_1)\leq& 2\EE_{\pi^*}[d\min\{H-h+1, 2B_1\sqrt{\frac{\alpha \log (B_2 k)}{N_{k,h}(s_h,a_h)}}\}].
\end{align*}
Because of Thm. \ref{thm:algO_regret_vs_algP_density}, on the event $\cECk$ and $\cEOk$, we further have:
\begin{align*}
    N_{k,h}(s_h,a_h) \geq& \frac{1}{2}\sum_{\pk=1}^k d^{\piO_\pk}(s_h,a_h) - \alpha \log(SAHk) \\
    \geq& \frac{1}{2}\sum_{\pk=1}^k d^{\pi^*_\pk}(s_h,a_h) - \alpha \log(SAHk) - \frac{1}{\Delta_{\min}}(C_1+\alpha C_2\log k)\\
    \geq& \frac{k}{2}d^{\pi^*}(s_h,a_h) - \alpha \log(SAHk) - \frac{1}{\Delta_{\min}}(C_1+\alpha C_2\log k)
\end{align*}
% Combining with Cond. \ref{cond:requirement_on_algO}, by applying Thm. \ref{thm:algO_regret_vs_algP_density}, we have with probability $1-2\delta_k$:
% \begin{align*}
%     N_{k,h}(s_h,a_h) \geq& \frac{1}{2}\sum_{\tk=1}^\nk d^{\pi_\tk}(s_h,a_h) - \log\frac{1}{\delta_k} \\
%     \geq& \frac{1}{2}\sum_{\tk=1}^\nk \Big(d^{\pi^*_\tk}(s_h,a_h) - \frac{1}{\Delta_{\min}} (V^*_1(s_1)-V^{\pi_\tk}_1(s_1)\Big)- \log\frac{1}{\delta_k}\\
%     \geq& \frac{1}{2}\sum_{\tk=1}^\nk d^{\pi^*_\tk}(s_h,a_h) - \frac{1}{\Delta_{\min}}\Big(C_1 + C_2 \log \frac{k}{\delta_k}\Big)- \log\frac{1}{\delta_k}\\
%     =& \blue{\frac{1}{2}k d^{\pi^*}(s_h,a_h) - \frac{1}{\Delta_{\min}}\Big(C_1 + C_2 \log \frac{k}{\delta_k}\Big)- \log\frac{1}{\delta_k}}
% \end{align*}
Now, we define that,
\begin{align*}
    \tau^{\pi^*}_{s_h,a_h} := & \inf_{t:\forall t' \geq t} \{\frac{1}{4}t d^{\pi^*}(s_h,a_h) \geq \alpha \log(SAHt) + \frac{1}{\Delta_{\min}}(C_1+\alpha C_2\log t)\}
\end{align*}
there must exists a constant $c_\tau$ independent with $C_1,C_2,\alpha, d^{\pi^*}(s_h,a_h)$ and $\Delta_{\min}$, such that:
\begin{align*}
    \forall h\in[H],s_h\in\cS_h,a_h\in\cA_h,\quad \tau^{\pi^*}_{s_h,a_h} \leq \btau^{\pi^*}_{s_h,a_h}:=c_\tau\frac{\alpha(C_1+C_2)}{d^{\pi^*}(s_h,a_h)\Delta_{\min}} \log \frac{\alpha SAH(C_1+C_2)}{d^{\pi^*}(s_h,a_h) \Delta_{\min}}.
\end{align*}
Easy to check that, for arbitrary $k \geq \btau^{\pi^*}_{s_h,a_h}$, on the good events, we can verify that $N_{k,h} \geq \frac{k}{4}d^{\pi^*}(s_h,a_h) \geq \frac{\btau^{\pi^*}_{s_h,a_h}}{4}d^{\pi^*}(s_h,a_h) \geq \frac{c_\tau}{4} > 0$, and as a result, we have:
\begin{align*}
    & V^*_1(s_1) - V_1^{\piE_k}(s_1) \\
    \leq& 2\EE_{\pi^*}\Big[\sum_{h=1}^H\Clip\Big[\min\{H-h+1, 2B_1\sqrt{\frac{\alpha \log (B_2 k)}{N_{k,h}(s_h,a_h)}}\}\Big|\epsClip\Big]\Big]\\
    \leq& 2\EE_{\pi^*}\Big[\sum_{h=1}^H\Clip\Big[\mathbb{I}[k < \btau^{\pi^*}_{s_h,a_h}]\}\cdot H + \mathbb{I}[k \geq \btau^{\pi^*}_{s_h,a_h}]\cdot B_1\sqrt{\frac{\alpha \log (B_2 k)}{kd^{\pi^*}(s_h,a_h)/4}}\Big|\epsClip\Big]\Big]
\end{align*}
\paragraph{Case 2: multiple optimal deterministic policies}
The discussion are similar. As a result of Thm. \ref{thm:existence_of_well_covered_optpi}, on the event $\cECk$ and $\cEOk$, we further have:
\begin{align*}
    N_{k,h}(s_h,a_h) \geq& \frac{k}{4}\cdot\max\{\frac{d^*_{h,\min}(s_h,a_h)}{(|\cZ_{h,\text{div}}|+1)H}, d^{\pi^*_{\text{cover}}}(s_h,a_h)\} - \alpha \log(SAHk) - \frac{1}{\Delta_{\min}} \Big(\sum_{k=1}^K V^*_1(s_1)-V^{\pi_k}_1(s_1)\Big) \\
    \geq& \frac{k}{4}\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h) - \alpha \log(SAHk) - \frac{1}{\Delta_{\min}}(C_1+\alpha C_2\log k)
\end{align*}
Similarly, we define that,
\begin{align*}
    \tau^{\pi^*_{\text{cover}}}_{s_h,a_h} := & \inf_{t:\forall t' \geq t} \{\frac{t}{8}\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h) \geq \alpha \log(SAHt) + \frac{1}{\Delta_{\min}}(C_1+\alpha C_2\log t)\}
\end{align*}
there must exists a constant $c'_\tau$ independent with $C_1,C_2,\alpha, \tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)$ and $\Delta_{\min}$, such that:
\begin{align*}
    \forall h\in[H],s_h\in\cS_h,a_h\in\cA_h,\quad \tau^{\pi^*_{\text{cover}}}_{s_h,a_h} \leq \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}:=c'_\tau\frac{\alpha(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)\Delta_{\min}} \log \frac{\alpha SAH(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h) \Delta_{\min}}.
\end{align*}
For arbitrary $k \geq \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}$, on the good events, we can verify that $N_{k,h} \geq \frac{k}{8}d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0$, and as a result, we have:
\begin{align*}
    & V^*_1(s_1) - V_1^{\piE_k}(s_1) \leq 2\EE_{\pi^*_{\text{cover}}}\Big[\sum_{h=1}^H\Clip\Big[\mathbb{I}[k < \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}]\}\cdot H + \mathbb{I}[k \geq \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}]\cdot B_1\sqrt{\frac{8\alpha \log (B_2 k)}{k\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)}}\Big|\epsClip'\Big]\Big]
\end{align*}
\end{proof}
Now, we are ready to prove the main theorem.
\ThmUBPVI*
\begin{proof}
Because the expectation and summation are linear, we have:
\begin{align*}
    \EE[\sum_{k=1}^K V^* - V^{\piE_k}] = \sum_{k=1}^K \EE[V^* - V^{\piE_k}]
\end{align*}
Therefore, in the following, we first provide an upper bound for each $\EE[V^* - V^{\piE_k}]$. Note that the expected regert at step $k$ can be upper bounded by:
\begin{align*}
    &\EE_{\algO, M, \algE}[V_1^*(s_1)-V^{\piE_k}_1(s_1)] \\
    =& \Pr(\cEBk\cap\cECk\cap\cEOk)\EE_{\algO, M, \algE}[V_1^*(s_1)-V^{\piE_k}_1(s_1)|\cEBk\cap\cECk\cap\cEOk]\\
    &+ \Pr(\cEBk^\complement\cup\cECk^\complement\cup\cEOk^\complement)\EE_{\algO, M, \algE}[V_1^*(s_1)-V^{\piE_k}_1(s_1)|\cEBk^\complement\cup\cECk^\complement\cup\cEOk^\complement]\\
    \leq& \Pr(\cEBk\cap\cECk\cap\cEOk)\EE_{\algO, M, \algE}[V_1^*(s_1)-V^{\piE_k}_1(s_1)|\cEBk\cap\cECk\cap\cEOk] + \frac{3H}{k^\alpha}
    % \\
    % \leq& 2\EE_{\pi^*}\Big[\sum_{h=1}^H\Clip\Big[\mathbb{I}[k < \btau^{\pi^*}_{s_h,a_h}]\}\cdot H + \mathbb{I}[k \geq \btau^{\pi^*}_{s_h,a_h}]\cdot B_1\sqrt{\frac{\alpha \log (B_2 k)}{kd^{\pi^*}(s_h,a_h)/4}}\Big|\epsClip\Big]\Big] + \frac{3H}{k^\alpha} \tag{Lemma \ref{thm:SubOpt_under_GoodEvents} and $V^*-V^\pi \leq H$}
\end{align*}
Easy to see that $\lim_{K\rightarrow \infty}\sum_{k=1}^K \frac{1}{k^\alpha} < \frac{\alpha}{\alpha - 1} < \infty$ as long as $\alpha > 1$, therefore, in the following, we mainly focus on the first part, and separately discuss its upper bound for the case when $|\Pi^*|=1$ or $|\Pi^*|>1$.
\paragraph{Case 1: $|\Pi^*|=1$ (Unique Optimal Policy)}
We use $\pi^*$ to denote the unique optimal policy and define:
\begin{align*}
    \tau^{\pi^*}_{s_h,a_h,\epsClip} := \inf_{t,\forall t' \geq t} \{B_1\sqrt{\frac{\alpha \log (B_2 t)}{td^{\pi^*}(s_h,a_h)/4}} < \epsClip\}
\end{align*}
Recall that $\epsClip:= \Delta_{\min}/(2H+2)$, it's easy to verify that, there exists a constant $c_{\text{Clip}}$ such that,
\begin{align*}
    \tau^{\pi^*}_{s_h,a_h,\epsClip} \leq \ttau^{\pi^*}_{s_h,a_h,\epsClip} := c_{\text{Clip}} \frac{\alpha H^2}{d^{\pi^*}(s_h,a_h)\Delta^2_{\min}} \log \frac{\alpha B_2 H}{d^{\pi^*}(s_h,a_h)\Delta_{\min}}
\end{align*}
Then, we have:
\begin{align*}
    \lim_{K\rightarrow \infty} \quad &\sum_{k=1}^K 2\EE_{\pi^*}\Big[\sum_{h=1}^H\Clip\Big[\mathbb{I}[k < \btau^{\pi^*}_{s_h,a_h}]\}\cdot H + \mathbb{I}[k \geq \btau^{\pi^*}_{s_h,a_h}]\cdot B_1\sqrt{\frac{\alpha \log (B_2 k)}{kd^{\pi^*}(s_h,a_h)/4}}\Big|\epsClip\Big]\Big]\\
    =&2\EE_{\pi^*}\Big[\sum_{h=1}^H\Big(\sum_{k=1}^{\btau^{\pi^*}_{s_h,a_h}} H+\sum_{k=\btau^{\pi^*}_{s_h,a_h}+1}^K \Clip\Big[B_1\sqrt{\frac{\alpha \log (B_2 k)}{kd^{\pi^*}(s_h,a_h)/4}}\Big|\epsClip\Big]\Big)\Big]\\
    \leq& 2\EE_{\pi^*}[\sum_{h=1}^H\sum_{k=1}^{\btau^{\pi^*}_{s_h,a_h}} H] + 2\EE_{\pi^*}\Big[\sum_{h=1}^H\int_{x=\btau^{\pi^*}_{s_h,a_h}}^{\ttau^{\pi^*}_{s_h,a_h,\epsClip}} B_1\sqrt{\frac{\alpha \log (B_2 x)}{xd^{\pi^*}(s_h,a_h)/4}} dx]\\
    \leq& 2\EE_{\pi^*}[\sum_{h=1}^H\sum_{k=1}^{\btau^{\pi^*}_{s_h,a_h}} H] + 2\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} B_1 \sqrt{4\alpha d^{\pi^*}(s_h,a_h)}\int_{x=\btau^{\pi^*}_{s_h,a_h}}^{\ttau^{\pi^*}_{s_h,a_h,\epsClip}} \sqrt{\frac{\log (B_2 x)}{x}}dx
\end{align*}
For the first part, we have:
\begin{align*}
    \EE_{\pi^*}[\sum_{h=1}^H\sum_{k=1}^{\btau^{\pi^*}_{s_h,a_h}} H] =& \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} d^{\pi^*}(s_h,a_h) \cdot H \cdot \btau^{\pi^*}_{s_h,a_h} \\
    \leq&c_\tau\frac{\alpha H(C_1+C_2)}{\Delta_{\min}} \cdot \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} \log \frac{\alpha SAH(C_1+C_2)}{d^{\pi^*}(s_h,a_h) \Delta_{\min}}
\end{align*}
For the second part, we have:
\begin{align*}
    & \EE_{\pi^*}\Big[\sum_{h=1}^H\int_{x=\btau^{\pi^*}_{s_h,a_h}}^{\ttau^{\pi^*}_{s_h,a_h,\epsClip}} B_1\sqrt{\frac{\alpha \log (B_2 x)}{xd^{\pi^*}(s_h,a_h)/4}} dx]\\
    \leq& \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} B_1 \sqrt{4\alpha d^{\pi^*}(s_h,a_h)}\int_{x=\btau^{\pi^*}_{s_h,a_h}}^{\ttau^{\pi^*}_{s_h,a_h,\epsClip}} \sqrt{\frac{\log (B_2 x)}{x}}dx\\
    \leq& 2\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} B_1 \sqrt{4\alpha d^{\pi^*}(s_h,a_h)}\cdot 2(\sqrt{\ttau^{\pi^*}_{s_h,a_h,\epsClip}\log B_2\ttau^{\pi^*}_{s_h,a_h,\epsClip}} - \sqrt{\btau^{\pi^*}_{s_h,a_h}\log B_2 \btau^{\pi^*}_{s_h,a_h}}) \tag{Lemma \ref{lem:compute_integral}}\\
    \leq & c_2 \frac{\alpha B_1 H}{\Delta_{\min}} \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} \log \frac{\alpha B_2 H}{d^{\pi^*}(s_h,a_h)\Delta_{\min}}
\end{align*}
where in the last step, we drop the term $-\sqrt{\btau^{\pi^*}_{s_h,a_h}\log B_2 \btau^{\pi^*}_{s_h,a_h}}$, and $c_2$ is a constant.

Combining the above results, we have:
\begin{align*}
&\EE_{\algO, M, \algE}[\sum_{k=1}^K V_1^*(s_1)-V^{\piE_k}_1(s_1)]\\
\leq& \sum_{k=1}^K \frac{3H}{k^\alpha} + c_\tau\frac{\alpha(C_1+C_2)}{\Delta_{\min}} \cdot \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} \log \frac{\alpha SAH(C_1+C_2)}{d^{\pi^*}(s_h,a_h) \Delta_{\min}} \\
&+ c_2\frac{\alpha B_1 H}{\Delta_{\min}} \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} \log \frac{\alpha B_2 H}{d^{\pi^*}(s_h,a_h)\Delta_{\min}} \\
\leq& \frac{3\alpha H}{\alpha - 1} + c_{\algE}\cdot \Big(\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} \frac{\alpha(C_1+C_2)}{\Delta_{\min}}\log \frac{\alpha SAH(C_1+C_2)}{d^{\pi^*}(s_h,a_h) \Delta_{\min}} + \frac{\alpha B_1 H}{\Delta_{\min}}\log \frac{\alpha B_2 H}{d^{\pi^*}(s_h,a_h)\Delta_{\min}}\Big)
\end{align*}
where $c_{\algE}$ is some constant.
\paragraph{Case 2: $|\Pi^*|>1$ (Non-Unique Optimal Policy)}
Similar to the discussion above, we define:
\begin{align*}
    \tau^{\pi^*_{\text{cover}}}_{s_h,a_h,\epsClip'} := \inf_{t,\forall t' \geq t} \{B_1\sqrt{\frac{8\alpha \log (B_2 t)}{t\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)}} < \epsClip'\}
\end{align*}
Recall that $\epsClip':= d_{\min}\Delta_{\min}/(2SAH)$, it's easy to verify that, there exists a constant $c_{\text{Clip}}$ such that,
\begin{align*}
    \tau^{\pi^*_{\text{cover}}}_{s_h,a_h,\epsClip'} \leq \ttau^{\pi^*_{\text{cover}}}_{s_h,a_h,\epsClip'} := c_{\text{Clip}} \frac{\alpha (SAH)^2}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)(d_{\min}\Delta_{\min})^2} \log \frac{\alpha B_2 SAH}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)d_{\min}\Delta_{\min}}
\end{align*}
Following a similar discussion, we have:
\begin{align*}
    \lim_{K\rightarrow \infty} \quad &\sum_{k=1}^K 2\EE_{\pi^*_{\text{cover}}}\Big[\sum_{h=1}^H\Clip\Big[\mathbb{I}[k < \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}]\}\cdot H + \mathbb{I}[k \geq \btau^{\pi^*_{\text{cover}}}_{s_h,a_h}]\cdot B_1\sqrt{\frac{8\alpha \log (B_2 k)}{k\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)}}\Big|\epsClip'\Big]\Big]\\
    \leq& 2\EE_{\pi^*_{\text{cover}}}[\sum_{h=1}^H\sum_{k=1}^{\btau^{\pi^*_{\text{cover}}}_{s_h,a_h}} H] + 2\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0}} B_1 \sqrt{8\alpha d^{\pi^*_{\text{cover}}}(s_h,a_h)}\int_{x=\btau^{\pi^*_{\text{cover}}}_{s_h,a_h}}^{\ttau^{\pi^*_{\text{cover}}}_{s_h,a_h,\epsClip'}} \sqrt{\frac{\log (B_2 x)}{x}}dx\\
    \leq& c'_\tau\frac{\alpha H(C_1+C_2)}{\Delta_{\min}} \cdot \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0}} \log \frac{\alpha SAH(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h) \Delta_{\min}}\\
    &+c_2' \frac{\alpha B_1 SAH}{d_{\min}\Delta_{\min}} \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0}} \log \frac{\alpha B_2 SAH}{d_{\min}\Delta_{\min}} \tag{Note that $\tilde{d}^{\pi^*_{\text{cover}}} \geq d^{\pi^*_{\text{cover}}}$}
\end{align*} 
Therefore, we have:
\begin{align*}
&\EE_{\algO, M, \algE}[\sum_{k=1}^K V_1^*(s_1)-V^{\piE_k}_1(s_1)]\\
\leq& \frac{3\alpha H}{\alpha - 1} + c'_{\algE}\cdot\Big(\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0}} \frac{\alpha(C_1+C_2)}{\Delta_{\min}}\log \frac{\alpha SAH(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)\Delta_{\min}} + \frac{\alpha B_1 SAH}{d_{\min}\Delta_{\min}}\log \frac{\alpha B_2 SAH}{d_{\min}\Delta_{\min}}\Big)
\end{align*}
\end{proof}

\begin{lemma}[Computation of Integral]\label{lem:compute_integral}
    Suppose $p \geq 1$, $b \geq a \geq e/p$, then we have:
    \begin{align*}
        \int_a^b \sqrt{\frac{\log px}{x}} dx \leq 2(\sqrt{b\log pb} - \sqrt{a\log pa})
    \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        \int_a^b \sqrt{\frac{\log px}{x}} dx \leq \int_a^b \frac{1}{\sqrt{x\log px}}+\sqrt{\frac{\log px}{x}} dx= 2\int_a^b (\sqrt{x\log px})' = 2(\sqrt{b\log pb} - \sqrt{a\log pa})
    \end{align*}
\end{proof}




\iffalse
\red{TODO: check more about this lemma}
\begin{lemma}[Corresponding to Lemma D.1 in \citep{simchowitz2019non}]
    Suppose the algorithm is pessimistic, we have (\red{we ignore the "strong pessimistic" for now and assume that $\alpha = 1$}), we have:
    \begin{align*}
        \Delta_h(s_h,a_h)\leq \surplus_{k,h}(s_h,a_h)+ \mP_h(s_h,a_h)\trans(V^*_{h+1}-\hV_{k,h+1}),\quad\forall s_h\in\cS_h,a_h\in\cA_h,h\in[H]
    \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        \Delta_h(s_h,a_h) =& V^*_h(s_h) - Q^*_h(s_h,a_h) \leq V^*_h(s_h) - \hQ_{k,h}(s_h,a_h)\\
        =&\surplus_{k,h}(s_h,a_h) + \mP_h(s_h,a_h)\trans(V^*_{h+1} - \hV_{k,h+1})
    \end{align*}
\end{proof}
Next, we will provide an upper bound for the r.h.s.

\begin{lemma}[Gap Clipping; Corresponding to Lemma D.3 in \citep{simchowitz2019non}]
    \begin{align*}
        V^*_h(s_h) - \ddot{V}^{*}_h(s_h) \leq \tilde{\surplus}_{k,h}(s_h, \pi^*)+(1+\frac{1}{H})\mP_h(s_h,\pi^*)\trans (V^*_1 - \ddot{V}^{*}_1)
    \end{align*}
    where we define:
    \begin{align*}
        \tilde{\surplus}_{k,h}(s_h,a_h) := {\rm Clip}[\surplus_{k,h}(s_h,a_h)|\epsClip \vee \frac{\Delta_h(s_h,a_h)}{4H}]
    \end{align*}
    % \begin{align*}
    %     \tilde{\surplus}_{k,h}(s_h,a_h) := {\rm Clip}[\surplus_{k,h}(s_h,a_h)|\epsClip \vee \frac{\Delta_h(s_h,a_h)}{4(\alpha_{s_h,a_h,h} H \vee 1)}] \leq {\rm Clip}[\surplus_{k,h}(s_h,a_h)|\frac{\Delta_{\min}}{2H} \vee \frac{\Delta_h(s_h,a_h)}{4H}]
    % \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        \Delta_h(s_h,a_h) \leq& \surplus_{k,h}(s_h,a_h) + \mP_h(s_h,a_h)\trans(V^*_{h+1}-\hV_{k,h+1}) \\
        \leq& \ddot{\surplus}_{k,h}(s_h,a_h) + \mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1}) + (H-h+2)\epsClip \tag{$\surplus \leq \ddot\surplus + \epsClip$ and Lemma \ref{lem:Vddot_and_V}}\\
        \leq& \ddot{\surplus}_{k,h}(s_h,a_h) + \mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1}) + \frac{\Delta_h(s_h,a_h)}{2}
        % \tag{\red{TODO we need to change the definition to $\epsClip=\Delta_{\min}/(2H+1)$}}
    \end{align*}
    which implies:
    \begin{align*}
        \ddot{\surplus}_{k,h}(s_h,a_h) + \mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1}) \geq \frac{\Delta_h(s_h,a_h)}{2}
    \end{align*}
    Similar to \citep{simchowitz2019non}, we consider two cases given a fixed $c\in(0,1]$, i.e. either $\ddot\surplus_{k,h}(s_h,a_h) \geq \frac{c}{2} \Delta_h(s_h,a_h)$ or otherwise,
    \begin{align*}
        \mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1}) \geq \frac{1-c}{c}\ddot\surplus_{k,h}(s_h,a_h)
    \end{align*}
    which implies that $\ddot\surplus_{k,h}(s_h,a_h) \leq \frac{c}{1-c}\mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1})$.
    Therefore,
    \begin{align*}
        \ddot\surplus_{k,h}(s_h,a_h) \leq& \ddot\surplus_{k,h}(s_h,a_h) \mathbb{I}[\ddot\surplus_{k,h}(s_h,a_h) \geq \frac{c}{2}\Delta_h(s_h,a_h)] \\
        &+ \frac{c}{1-c}\mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1}) \mathbb{I}[\ddot\surplus_{k,h}(s_h,a_h) < \frac{c}{2}\Delta_h(s_h,a_h)] \\
        \leq&\ddot\surplus_{k,h}(s_h,a_h) \mathbb{I}[\ddot\surplus_{k,h}(s_h,a_h) \geq \frac{c}{2}\Delta_h(s_h,a_h)] +  \frac{c}{1-c}\mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1})
    \end{align*}
    which implies:
    \begin{align*}
        &\ddot\surplus_{k,h}(s_h,a_h) + \mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1})\\
        \leq& \ddot\surplus_{k,h}(s_h,a_h) \mathbb{I}[\ddot\surplus_{k,h}(s_h,a_h) \geq \frac{c}{2}\Delta_h(s_h,a_h)] + (1+\frac{c}{1-c})\mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1})
    \end{align*}
    By choosing $c=1/(2H)$, we have:
    \begin{align*}
        \ddot\surplus_{k,h}(s_h,a_h) + \mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1}) \leq \tilde{\surplus}_{k,h}(s_h,a_h) + (1+\frac{1}{H})\mP_h(s_h,a_h)\trans(V^*_{h+1}-\ddot{V}^*_{k,h+1})
    \end{align*}
\end{proof}
Based on Lemma above, we have:
\begin{align*}
    V^*_1(s_1) - V^{\pi_k}_1(s_1)\leq& 2 V^*_1(s_1) - \ddot{V}^{*}_1(s_1) \leq 2\EE_{\pi^*}[\sum_{h=1}^H (1+\frac{1}{H})^h \tilde{\surplus}_{k,h}(s_h,a_h)]\\
    \leq& 2e\EE_{\pi^*}[\sum_{h=1}^H \tilde{\surplus}_{k,h}(s_h,a_h)]\\
    =&2e\sum_{h=1}^H \sum_{s_h,a_h} d^{\pi^*}(s_h,a_h)\tilde{\surplus}_{k,h}(s_h,a_h)
\end{align*}
\fi

==> arxiv /Gap_Agnostic_UCB.tex <==
\section{Analysis for Bandit Setting}\label{appx:analysis_for_bandit_setting}


% \subsection{Another Results}
% \begin{proof}
%     \begin{align*}
%         &\Pr(N_{i^*}(k) < N_i(k) / 4) \\
%         \leq& \sum_{k_0=4 N_{i^*}(k)}^{k}\Pr(\{N_{i^*}(k)\leq N_i(k_0)/4\}\cap \{N_{i^*}(k)\geq N_i(k_0-1)/4\}) \\
%         \leq&\sum_{k_0=4 N_{i^*}(k)}^{k}\Pr(\{N_{i^*}(k)\leq N_i(k_0)/4\}\cap \{N_{i^*}(k)\geq N_i(k_0-1)/4\}\\
%         &\qquad\qquad\cap\{\hat\mu_{i^*}(k_0)+\sqrt{\frac{2\alpha f(k_0-1)}{N_{i^*}(k_0)}} \leq \hat\mu_{i}(k_0)+\sqrt{\frac{2\alpha f(k_0-1)}{N_{i}(k_0)}}\})\\
%         =&\sum_{k_0=4 N_{i^*}(k)}^{k}\Pr(\{N_{i^*}(k)\leq N_i(k_0)/4\}\cap \{N_{i^*}(k)\geq N_i(k_0-1)/4\} \\
%         &\qquad\qquad \cap\{\hat\mu_{i^*}(k_0)-\mu_{i^*}+\Delta_i+\sqrt{\frac{2\alpha f(k_0-1)}{N_{i^*}(k_0)}} \leq \hat\mu_{i}(k_0)-\mu_i+\sqrt{\frac{2\alpha f(k_0-1)}{N_{i}(k_0)}}\})\\
%         \leq&\sum_{k_0=4 N_{i^*}(k)}^{k}\Pr(\{N_{i^*}(k)\leq N_i(k_0)/4\}\cap \{N_{i^*}(k)\geq N_i(k_0-1)/4\} \\
%         &\qquad\qquad \cap\{\hat\mu_{i^*}(k_0)-\mu_{i^*}+\Delta_i\leq \hat\mu_{i}(k_0)-\mu_i-\sqrt{\frac{2\alpha f(k_0-1)}{N_{i}(k_0)}}\}) \\
%         \leq& \sum_{k_0=4 N_{i^*}(k)}^{k}\Pr(\{N_{i^*}(k)\leq N_i(k_0)/4\}\cap \{N_{i^*}(k)\geq N_i(k_0-1)/4\}\cap\{0\leq \hat\mu_{i}(k_0)-\mu_i-\sqrt{\frac{2\alpha f(k_0-1)}{N_{i}(k_0)}}\}) \\
%         &\quad\quad+\Pr(\{N_{i^*}(k)\leq N_i(k_0)/4\}\cap \{N_{i^*}(k)\geq N_i(k_0-1)/4\}\cap\{\hat\mu_{i^*}(k_0)-\mu_{i^*}+\Delta_i\leq 0\})
%     \end{align*}
% \end{proof}


\subsection{The Optimality of $\algO$ in Alg \ref{alg:UCB_Explore_LCB_Exploit}}\label{sec:optimality_of_algO}
From Theorem 8.1 of \citep{lattimore2020bandit}, 
we can show the following guarantee for the UCB algorithm in Alg \ref{alg:UCB_Explore_LCB_Exploit} with revised bonus function:
\begin{align*}
    \EE[\sum_{k=1}^K \mu_1- \mu_{\piO_k}] \leq& \sum_{i: \Delta_i > 0} \Delta_i + \frac{1}{\Delta_i}(8\alpha\log f(K) + 8\sqrt{\pi \alpha \log f(K)} + 28)\\
    =&O(\sum_{i:\Delta_i > 0}\frac{\alpha}{\Delta_i} \log AK)
    % =O(\sum_{i:\Delta_i > 0}\frac{\alpha}{\Delta_i} \log K)
\end{align*}
where we assume $K \geq A$. Since $\alpha$ is just at the constant level, the above regret still matches the lower bound.

\subsection{Analysis for LCB}
\paragraph{Outline} 
In this section, we establish regret bound for Alg. \ref{alg:UCB_Explore_LCB_Exploit}. We first provide the proof of two key Lemma: Lem. \ref{lem:blessing_of_pessimism} and Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar}. After that, in Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar}, we try to combine the above two results and prove that for those arm $i$ with $\Delta_i > 0$, when $k$ is large enough, we are almost sure (with high probability) that LCB will not take arm $i$.
Finally, we conclude this section with the proof of Thm. \ref{thm:total_regret_UCB_LCB}.

\paragraph{Definition of $c_f$}
Under the choice $f(k)=1+16A^2(k+1)^2$, we use $c_f$ to denote the minimal positive constant independent with $\alpha, A$ and arbitrary $\Delta_i$ with $\Delta_i > 0$, such that
\begin{align*}
    \forall~\Delta_i > 0, \forall \scalar \in [1, 4A],\quad \text{as long as}\quad  k \geq& c_f \frac{\alpha \scalar}{\Delta_i^2} \log (1+\frac{\alpha A}{\Delta_i}), \quad \\
    \text{we have}\quad k \geq& \frac{32\alpha \scalar}{\Delta_i^2} \log f(k) \numberthis\label{eq:def_c_f_new}
\end{align*}


% For each $\Delta_i > 0$, we define $\bar{i}$ to be:
% as long as $\Delta_i \neq \Delta_{\min}$, we can find an arm $\bar{i}$ (it's possible that $\bar{i}=i$), such that 
% \begin{align*}
%     \bar{i}:= \arg\min_{i \in \cA} \Delta_{\bar{i}},\quad s.t.\quad \Delta_{\bar{i}} \geq \Delta_i / 2
% \end{align*}
% Note that it's possible that $\bar{i}=i$. 

\LemBlessingLCB*
\begin{proof}
    \begin{align*}
        & \Pr(\{i = \piE_k\}\cap \{\Delta_j < \Delta_i\} \cap \{N_j(k) \geq \frac{8\alpha\log f(k)}{(\Delta_j - \Delta_i)^2}\})\\
        \leq & \Pr(\{\hat\mu_i(k)-\sqrt{\frac{2\alpha \log f(k)}{N_i(k)}} \geq \hat\mu_{j}(k)-\sqrt{\frac{2\alpha \log f(k)}{N_{j}(k)}}\}\cap \{\Delta_j < \Delta_i\} \cap \{N_j(k) \geq \frac{8\alpha\log f(k)}{(\Delta_j - \Delta_i)^2}\}) \\
        = & \Pr(\{\hat\mu_i(k)-\mu_i-\sqrt{\frac{2\alpha \log f(k)}{N_i(k)}} \geq \hat\mu_{j}(k)-\mu_j + (\Delta_j - \Delta_i)-\sqrt{\frac{2\alpha \log f(k)}{N_{j}(k)}}\}\\
        &\quad\quad\cap \{\Delta_j < \Delta_i\} \cap \{N_j(k) \geq \frac{8\alpha\log f(k)}{(\Delta_j - \Delta_i)^2}\})\\
        \leq& \Pr(\{\hat\mu_i(k)-\mu_i-\sqrt{\frac{2\alpha \log f(k)}{N_i(k)}} \geq \hat\mu_{j}(k)-\mu_j + \sqrt{\frac{2\alpha \log f(k)}{N_{j}(k)}}\}\cap \{\Delta_j < \Delta_i\} \cap \{N_j(k) \geq \frac{8\alpha\log f(k)}{(\Delta_j - \Delta_i)^2}\})\\
        \leq&\Pr(\{\hat\mu_i(k)-\mu_i-\sqrt{\frac{2\alpha \log f(k)}{N_i(k)}} \geq \hat\mu_{j}(k)-\mu_j + \sqrt{\frac{2\alpha \log f(k)}{N_{j}(k)}}\})\\
        \leq& \Pr(\{\hat\mu_i(k)-\mu_i-\sqrt{\frac{2\alpha \log f(k)}{N_i(k)}} \geq 0\}) + \Pr(\{0 \geq \hat\mu_{j}(k)-\mu_j + \sqrt{\frac{2\alpha \log f(k)}{N_{j}(k)}}\}) \\
        \leq& 2/f(k)^\alpha \leq 2/k^{2\alpha}
    \end{align*}
    where the last but two step is because of the Azuma-Hoeffding's inequality.
\end{proof}

% \input{OldBound}
\input{NewBound}


==> arxiv /LSVI-LCB_and_LSVI-UCB.tex <==

\section{Some Guarantees}
Linear setting as an example. 
\paragraph{Pessimistic LSVI-UCB}
Suppose we run PEVI in \citep{jin2021pessimism} with a given dataset $D$, we have:
\begin{align*}
    V^* - V^{\bpi_k} \leq 2\beta \EE_{\pi^*}[\sum_{h=1}^H \sqrt{\phi(s_h,a_h)\trans\Sigma_h^{-1}\phi(s_h,a_h)}]:=\Delta_{P,k}
\end{align*}
\paragraph{Optimistic LSVI-UCB}
Suppose we run LSVI-UCB in \citep{jin2020provably} with a given dataset $D$, we have:
\begin{align*}
    V^* - V^{\pi_k} \leq 2\beta \EE_{\pi_k}[\sum_{h=1}^H \sqrt{\phi(s_h,a_h)\trans\Sigma_h^{-1}\phi(s_h,a_h)}]:=\Delta_{O,k}
\end{align*}

\paragraph{Informal Comparison between $\Delta_O$ and $\Delta_P$}
The gap between $\Delta_O$ and $\Delta_P$ should be instance-dependent. Intuitively, it depend on how often $Alg^O$ select policies $\pi_k$ which has non-trivial overlaps with $\pi^*$. 

Take the finite-arm bandit problem as an example. If all the arms are BeRegret(0.5) except that the optimal one is BeRegret(0.5+$\epsilon$), then $\Delta_P \approx \Delta_O$. However, as long as we modify one arm from BeRegret(0.5) to Ber (0.4), the difference is clear.

\begin{proposition}[Informal (To check later)]
In the multi-arm bandit problem, suppose we have $\mu_1 \geq \mu_2 \geq...\geq \mu_A$. Denote $\Delta_i = \mu_i - \mu_1.\forall i \geq 2$. We should have:
\begin{align*}
    \sum_{k=1}^K \Delta_{O,k} - \Delta_{P,k} \approx \sum_{i=2}^A \frac{\log K}{2\Delta_i}
\end{align*}
however...
\begin{align*}
    \sum_{k=1}^K \Delta_{O,k} \approx \sum_{i=2}^A \frac{\log K}{\Delta_i}
\end{align*}
which means the improvement is at the constant level...
\end{proposition}

\paragraph{Does there exist other methods to further reduce the regret of $Alg^P$?}

==> arxiv /NewBound.tex <==
\LemLBofNiNew*
\begin{proof}
    We choose $c_f$ defined in Eq.\eqref{eq:def_c_f_new} to be the constant $c$ in this Lemma.

    The key idea of the proof is that, because $N_i(k) \leq k$ for all $k$, if $N_i(k) \geq \lceil k / \scalar \rceil $, there must exists an iteration $\tk$ between $\lceil k/\scalar \rceil - 1$ and $k$, such that $\{N_i(\tk)=\lceil k/\scalar \rceil-1\}\cap \{N_i(\tk)=\lceil k/\scalar \rceil\}$ (i.e. $\tk$ is the time step that UCB takes arm $i$ for the $\lceil k/\scalar \rceil$-th time). Therefore, for arbitrary fixed $\lambda \in [1, A^2]$, when $k \geq \scalar + c_f \cdot \frac{\alpha \scalar}{\Delta_i^2}\log(1+\frac{\alpha \scalar}{\Delta_{\min}})$, we have:

    \begin{align*}
        &\Pr(N_i(k) \geq k/\scalar)=\Pr(N_i(k) \geq \lceil k/\scalar \rceil) \\
        =&\sum_{\tilde{k}=\lc k/\scalar \rc-1}^{k-1} \Pr(\{N_i(\tilde{k})=\lc k/\scalar \rc-1,N_i(\tilde{k}+1)=\lc k/\scalar \rc\}\cap \{\hat{\mu}_{i^*}(\tilde{k})+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_{i^*}(\tilde{k})}} \leq \hat\mu_i(\tilde{k})+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_i(\tilde{k})}}\}) \tag{Union bound.}\\
        =&\sum_{\tilde{k}=\lc k/\scalar \rc-1}^{k-1} \Pr(\{N_i(\tilde{k})=\lc k/\scalar \rc-1,N_i(\tilde{k}+1)=\lc k/\scalar \rc\}\\
        &\quad\quad\cap \{\hat{\mu}_{i^*}(\tilde{k})-\mu_{i^*}+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_{i^*}(\tilde{k})}} \leq \hat\mu_i(\tilde{k})-\mu_i-\Delta_i+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_i(\tilde{k})}}\}) \tag{Subtract $\mu_{i^*}$ at both sides}\\
        \leq& \sum_{\tilde{k}=\lc k/\scalar \rc-1}^{k-1} \Pr(\{N_i(\tilde{k})=\lc k/\scalar-1 \rc,N_i(\tilde{k}+1)=\lc k/\scalar \rc\}\cap\{\hat{\mu}_{i^*}(\tilde{k})-\mu_{i^*}+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_{i^*}(\tilde{k})}}\leq 0\})\\
        &\quad + \Pr(\{N_i(\tilde{k})=\lc k/\scalar \rc-1),N_i(\tilde{k})=\lc k/\scalar \rc+1)\}\cap\{0 \leq \hat\mu_i(\tilde{k})-\mu_i-\Delta_i+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_i(\tilde{k})}}\})\numberthis\label{eq:med_step_1}\\
        \leq& \sum_{\tilde{k}=\lc k/\scalar \rc-1}^{k-1} \Pr(\{\hat{\mu}_{i^*}(\tilde{k})-\mu_{i^*}+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_{i^*}(\tilde{k})}}\leq 0\})\\
        &\quad + \Pr(\{N_i(\tilde{k})=\lc k/\scalar \rc-1),N_i(\tilde{k}+1)=\lc k/\scalar \rc)\}\cap\{0 \leq \hat\mu_i(\tilde{k})-\mu_i-\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_i(\tilde{k})}}\}) \tag{Under our choice of $k$, and $N_i(\tilde{k})=\lc k/\scalar\rc-1$, $\frac{\log f(\tilde{k})}{N_i(\tilde{k})} \leq \frac{\log f(k)}{ k/\scalar - 1}\leq \frac{\Delta_i^2}{8\alpha}$}\\
        \leq&\sum_{\tilde{k}=\lc k/\scalar \rc-1}^{k-1} \Pr(\{\hat{\mu}_{i^*}(\tilde{k})-\mu_{i^*}+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_{i^*}(\tilde{k})}}\leq 0\}) + \Pr(\{0 \leq \hat\mu_i(\tilde{k})-\mu_i-\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_i(\tilde{k})}}\})\\
        \leq& \sum_{\tilde{k}=\lc k/\scalar \rc-1}^{k-1} \frac{2}{f(\tilde{k})^{\alpha}} \tag{Azuma-Hoeffding Inequality}\\
        \leq& \frac{2k}{f(k/\scalar-1)^{\alpha}} = \frac{2k}{(16A^2k^2/\scalar^2+1)^{\alpha}}\leq \frac{2}{k^{2\alpha-1}} \tag{$\scalar\in[1, 4A]$}
    \end{align*}
    where the step \eqref{eq:med_step_1} is because:
    \begin{align*}
        &\{\hat{\mu}_{i^*}(\tilde{k})-\mu_{i^*}+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_{i^*}(\tilde{k})}} < \hat\mu_i(\tilde{k})-\mu_i-\Delta_i+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_i(\tilde{k})}}\}\\
        \in& \{0 < \hat\mu_i(\tilde{k})-\mu_i-\Delta_i+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_i(\tilde{k})}}\} \cup \{\hat{\mu}_{i^*}(\tilde{k})-\mu_{i^*}+\sqrt{\frac{2\alpha \log f(\tilde{k})}{N_{i^*}(\tilde{k})}}\leq 0\}
    \end{align*}
\end{proof}

\begin{lemma}\label{lem:combining_UCB_with_LCB_new}
    Given an arm $i$, we separate all the arms into two parts depending on whether its gap is larger than $\Delta_i$ and define $\Gl_i:=\{\iota|\Delta_\iota > \Delta_i / 2\}$ and $\Gu_i:=\{\iota|\Delta_\iota \leq \Delta_i / 2\}$.
    With the choice that $f(k)=1+16A^2(k+1)^2$, there is a constant $c$, such that for arbitrary $i$ with $\Delta_i > 0$, for the LCB algorithm in Alg \ref{alg:UCB_Explore_LCB_Exploit}, we have:
    \begin{align}
        \Pr(i = \piE_k) \leq 2/k^{2\alpha}+2A/k^{2\alpha-1},\quad\forall k \geq k_i := 8\alpha c\Big(\sum_{\iota \in \Gl_i} \frac{1}{\Delta_\iota^2} + \frac{4|\Gu_i|}{\Delta_i^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}})\label{eq:def_ki}
    \end{align}
    where $c$ is the constant considered in Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar} (i.e. $c_f$ defined in Eq.\eqref{eq:def_c_f_new}).
\end{lemma}
\begin{proof}
    % Recall the $c$ considered in Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar}, given an arm $i$, we define:
    % \begin{align}
    %     k_{i}:=& \alpha c\Big(\sum_{\iota \in \Gl_i} \frac{1}{\Delta_\iota^2} + (1+\sum_{\iota \in \Gl_i} \frac{4}{\Delta_i^2})\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}) \\
    %     =& \alpha c\Big(\sum_{\iota \in \Gl_i} \frac{1}{\Delta_\iota^2} + (|\Gu_i|+1) \frac{4}{\Delta_i^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}})\label{eq:def_ki}
    % \end{align}
    We want to remark that the constants in the definition of $k_i$ (i.e. 8 in ``$8\alpha c$'' and 4 in ``''$4|\Gu_i|$'') can be replaced by others, but we choose them carefully in order to make sure some steps in the proof of this Lemma and Thm. \ref{thm:total_regret_UCB_LCB} can go through.

    The main idea of the proof is to use Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar} to show that, for those arm $i$ with $\Delta_i > 0$, when $k \geq k_i$, $N_\iota(k)$ will be small for those $\iota \in \Gl_i$. As a result, there must exist an arm $j \in \Gu_i$, such that $N_j(k)$ is large than the threshold considered in Lem. \ref{lem:blessing_of_pessimism} and therefore, with high probability, arm $i$ will not be preferred.

    First, we try to apply Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar} to upper bound the quantity $N_j(k)$ for those arm $j\in \Gl_i$.
    For each $j\in \Gl_i$, 
    we define the following quantity, which measures the magnitude of $1/\Delta_j^2$ with $k$:
    % we define the following quantity, which roughly captures the magnitude of $\Delta_j$ comparing with arms no less than $\Delta_i$.
    \begin{align*}
        \gamma_{k,j} := \frac{k}{\frac{8\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})}.
    \end{align*}
    We only consider $k \geq k_i$, where we always have $\gamma_{k,j} \geq 1$ based on the definition of $k_i$.

    Next, we separately consider two cases depending on whether $\gamma_{k,j} > 2A$ or not. 

    \textbf{Case 1: $\gamma_{k,j} > 2A$}: In this case, $\Delta_j$ is relatively large (or say more sub-optimal) comparing with iteration $k$. 
    For arbitrary $k \geq k_{i}$, we have
    \begin{align*}
        k =& \gamma_{k,j}\cdot \frac{8\alpha c}{\Delta_j^2 }\log(1+\frac{\alpha A}{\Delta_{\min}}) \geq 2A\cdot \frac{8\alpha c}{\Delta_j^2 }\log(1+\frac{\alpha A}{\Delta_{\min}}) \geq 2A + \frac{2\alpha c A}{\Delta_i^2} \log(1+\frac{\alpha A}{\Delta_{\min}}).
    \end{align*}
    which implies that $k$ satisfying the condition of applying Lemma \ref{lem:upper_bound_of_Nk_geq_k_div_scalar} with $\scalar = 2A$, and we can conclude that:
    $$
    \Pr(N_k(j) \geq \frac{k}{2A}) \leq \frac{2}{k^{2\alpha-1}}.
    $$
    % where the first inequality is because 
    % \begin{align*}
    %     k \geq k_i = \gamma_{k,j}\cdot \frac{8\alpha c_f}{\Delta_j^2 }\log(1+\frac{\alpha A}{\Delta_{\min}}) \geq A^2\cdot \frac{8\alpha c_f}{\Delta_j^2 }\log(1+\frac{\alpha A}{\Delta_{\min}})
    % \end{align*}
    % \begin{align*}
    %     \frac{k}{A^2} \geq \frac{k_{i}}{A^2} \geq \frac{8\alpha}{\Delta_j^2}
    %     \log(1+\frac{\alpha A}{\Delta_{\min}})
    % \end{align*}
    % and the second inequality results from applying Lem \ref{lem:upper_bound_of_Nk_geq_k_div_scalar} with condition $k\geq k_{i} \geq A^2 + c_f \cdot \frac{\alpha A^2}{\Delta_j^2}\log (1+\frac{2\alpha A^2}{\Delta_{\min}})$.

    \textbf{Case 2: $\gamma_{k,j} \leq 2A$}: Note that
    \begin{align*}
        \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}}) = \frac{k}{2\gamma_{k,j}}.
    \end{align*}
    Since $2\gamma_{k,j}$ locates in the interval $[1,4A]$ and:
    \begin{align*}
        k =& \gamma_{k,j}\cdot \frac{8\alpha c}{\Delta_j^2 }\log(1+\frac{\alpha A}{\Delta_{\min}})\geq 2\gamma_{k,j} + 2\gamma_{k,j}\cdot \frac{\alpha c}{\Delta_j^2} \log(1+\frac{\alpha A}{\Delta_{\min}})
    \end{align*}
    which satisfies the condition of applying Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar} with $\scalar = 2\gamma_{k,j}$. Therefore, we have:
    \begin{align}
        \Pr(N_k(j)\geq \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) = \Pr(N_k(j)\geq \frac{k}{2\gamma_{k,j}}) \leq \frac{2}{k^{2\alpha-1}}
    \end{align}
    Combining the above two cases, we can conclude that, for arbitrary $j \in \Gl_i$, 
    $$
    \Pr(N_j(k) \geq \frac{k}{2A} + \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) \leq \min\{ \Pr(N_j(k) \geq \frac{k}{2A}), \Pr(N_j(k) \geq \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}}))\} \leq \frac{2}{k^{2\alpha-1}}
    $$
    which reflects that with high probability, $\sum_{j\in \Gl_i} N_j(k)$ is small:
    \begin{align*}
        &\Pr(\sum_{j\in\Gl_i} N_j(k) \geq \frac{k}{2} + \sum_{j \in \Gl_i} \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) \\
        \leq & \sum_{j\in\Gl_i} \Pr(N_j(k)\geq \frac{k}{2|\Gl_i|} + \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) \tag{$P(a+b\leq c+d)\leq P(a\leq c) + P(b \leq d)$}\\
        \leq & \sum_{j\in\Gl_i} \Pr(N_j(k)\geq \frac{k}{2A} + \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) \tag{$|\Gl_i|\leq A$}\\
        \leq& \frac{2|\Gl_i|}{k^{2\alpha-1}}\leq \frac{2A}{k^{2\alpha-1}}
    \end{align*}
    Since $\sum_{j\in \Gu_i} N_j(k) + \sum_{j\in\Gl_i} N_j(k) = k$, and note that,
    \begin{align*}
        k - (\frac{k}{2} + \sum_{j\in \Gl_i} \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) = \frac{k}{2} - \sum_{j\in \Gl_i} \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}}) = \frac{16\alpha c|\Gu_i|}{\Delta_i^2}\log(1+\frac{\alpha A}{\Delta_{\min}})
    \end{align*}
    we have:
    \begin{align*}
        &\Pr(\sum_{j\in \Gu_i} N_j(k) \leq \frac{16\alpha c|\Gu_i|}{\Delta_i^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) \\
        % =& \Pr(\sum_{j\in \Gl_i} N_j(k) \geq k- \frac{\alpha c|\Gu_i|}{\Delta_i^2}\log(1+\frac{\alpha A}{\Delta_{\min}}))\\
        =& \Pr(\sum_{j\in\Gl_i} N_j(k) \geq \frac{k}{2} + \sum_{j \in \Gl_i} \frac{4\alpha c}{\Delta_j^2}\log(1+\frac{\alpha A}{\Delta_{\min}})) \\
        % \tag{$8\alpha c\cdot \frac{4|\Gu_i|}{\Delta_i^2}\log(1+\frac{\alpha A}{\Delta_{\min}}) \leq \frac{k_i}{2} \leq \frac{k}{2}$}
        \leq&\frac{2A}{k^{2\alpha-1}}
    \end{align*}
    Therefore, w.p, $1-\frac{2A}{k^{2\alpha-1}}$, there exists $j\in \Gu_i$, such that 
    \begin{align*}
        N_j(k) \geq \frac{1}{|\Gu_i|}\sum_{j\in \Gu_i} N_j(k) \geq \frac{16\alpha c}{\Delta_i^2}\log(1+\frac{\alpha A}{\Delta_{\min}}).
    \end{align*}
    Recall our choice of $c$ (Eq.\eqref{eq:def_c_f_new}), the above implies that:
    \begin{align}
        N_j(k) \geq \frac{32\alpha \log f(k)}{\Delta_i^2}.\label{eq:lower_bound_Gupper}
    \end{align}
    Therefore,
    \begin{align*}
        \Pr(\{i = \piE_k\}\cap\{k \geq k_{i}\})\leq & \Pr(\{i = \piE_k\}\cap\{k \geq k_{i}\}\cap\{\exists j \in \Gu_i: N_j(k) \geq \frac{32\alpha \log f(k)}{\Delta_i^2}\}) \\
        &+ \Pr(\{k \geq k_{i}\}\cap \neg \{\exists j \in \Gu_i: N_j(k) < \frac{32\alpha\log f(k)}{\Delta_i^2}\}) \\\leq & \Pr(\{i = \piE_k\}\cap\{k \geq k_{i}\}\cap\{\exists j \in \Gu_i: N_j(k) \geq \frac{32\alpha \log f(k)}{\Delta_i^2}\}) + \frac{2A}{k^{2\alpha-1}} \tag{Eq.\eqref{eq:lower_bound_Gupper}}\\
        \leq & \Pr(\{i = \piE_k\}\cap\{k \geq k_{i}\}\cap\{\exists j \in \Gu_i:  N_j(k) \geq \frac{8\alpha \log f(k)}{(\Delta_j-\Delta_j)^2}\}) + \frac{2A}{k^{2\alpha-1}} \\
        % \leq& \Pr(\{k \geq k_{i}\}\cap\{\exists j \in \Gu_i:  N_j(k) \geq \frac{8\alpha \log f(k)}{(\Delta_j-\Delta_j)^2}\}) + \frac{2A}{k^{2\alpha-1}} \\
        \leq & \frac{2}{k^{2\alpha}}+ \frac{2A}{k^{2\alpha-1}} \tag{Lem. \ref{lem:blessing_of_pessimism}}
    \end{align*}
\end{proof}

\begin{lemma}[Integral Lemma]\label{lem:integral_lem}
    For arbitrary $k_0 \geq 1$ and $\beta > 1$, we have:
    \begin{align*}
        \sum_{k=k_0+1}^\infty \frac{1}{k^\beta} \leq \int_{k_0}^\infty \frac{1}{x^\beta} dx \leq \frac{1}{(\beta-1)k_0^{\beta-1}} 
    \end{align*}
\end{lemma}


\ThmLCBRegret*
\begin{proof}
    Recall the definition of $k_i$ in Eq.\eqref{eq:def_ki} in Lem. \ref{lem:combining_UCB_with_LCB_new} above. For $i \geq 2$, if $\Delta_i \neq \Delta_{i-1}$, we have:
    \begin{align*}
        k_i - k_{i-1} =& \alpha c\Big(\sum_{\iota \in \Gl_i} \frac{8}{\Delta_\iota^2} - \sum_{\iota \in \Gl_{i-1}} \frac{8}{\Delta_\iota^2} + \frac{32|\Gu_i|}{\Delta_i^2} - \frac{32|\Gu_{i-1}|}{\Delta_{i-1}^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}) \\
        \leq & \alpha c\Big((|\Gl_i| - |\Gl_{i-1}|)\frac{32}{\Delta_{i}^2} + \frac{32|\Gu_i|}{\Delta_i^2} - \frac{32|\Gu_{i-1}|}{\Delta_{i-1}^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}) \tag{$\forall \iota \in \Gl_i \setminus \Gl_{i-1}$, we have $1/\Delta^2_\iota\leq 4/\Delta^2_{i}$}\\
        \leq & \alpha c\Big((|\Gu_{i-1}| - |\Gu_{i}|)\frac{32}{\Delta_{i}^2} + \frac{32|\Gu_i|}{\Delta_i^2} - \frac{32|\Gu_{i-1}|}{\Delta_{i-1}^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}) \tag{$|\Gu_{i-1}| + |\Gl_{i-1}|=|\Gu_{i}| + |\Gl_{i}|=A$}\\
        \leq&32\alpha c|\Gu_{i-1}|\Big(\frac{1}{\Delta_i^2}- \frac{1}{\Delta_{i-1}^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}).
    \end{align*}
    and if $\Delta_i = \Delta_{i-1}$, we also have:
    \begin{align*}
        k_i - k_{i-1} = 0 \leq 32\alpha c|\Gu_{i-1}|\Big(\frac{1}{\Delta_i^2}- \frac{1}{\Delta_{i-1}^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}).
    \end{align*}
    Moreover, for $i=1$, with the extended definition that $\Delta_0 = \infty$ (so that $1/\Delta_0^2=0$) and $|\Gu_0|=A$, we also have:
    \begin{align*}
        k_1 :=& 8\alpha c\Big(\sum_{\iota \in \Gl_1} \frac{1}{\Delta_\iota^2} + \frac{4|\Gu_1|}{\Delta_1^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}) \\
        \leq& 8\alpha c\Big(\sum_{\iota \in \Gl_1} \frac{4}{\Delta_1^2} + \frac{4|\Gu_1|}{\Delta_1^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}) \\
        =& \frac{32\alpha c A}{\Delta_1^2}\log(1+\frac{\alpha A}{\Delta_{\min}})\\
        =& 32\alpha c |\Gu_0|(\frac{1}{\Delta_1^2}-\frac{1}{\Delta_0^2})\log(1+\frac{\alpha A}{\Delta_{\min}}).
    \end{align*}
    % By extending the definition to $|\Gu_0| = A$ and $\Delta_0 = \infty$
    % , we also have:
    % \begin{align}
    %     k_1 - k_0 = k_1 = 32\alpha c|\Gu_{0}|\Big(\frac{1}{\Delta_i^2}- \frac{1}{\Delta_{i-1}^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}})
    % \end{align}
    Therefore, we have (we denote $k_A := \infty$ and $k_0:=0$):
    \begin{align*}
        \lim_{K \rightarrow \infty} \Regret_K(\algE) =& \sum_{k=1}^\infty \sum_{j:\Delta_j > 0} \Pr(j = \piE_k) \Delta_j \\
        =& \sum_{i=1}^A\sum_{k=k_{{i}-1}+1}^{k_{{i}}} \sum_{\Delta_j > 0} \Pr(j = \piE_k) \Delta_j \\
        =& \sum_{i=1}^A\sum_{k=k_{{i}-1}+1}^{k_{{i}}} \Big(\sum_{\Delta_j \geq \Delta_{i-1}} \Pr(j = \piE_k)\Delta_j + \sum_{\Delta_j < \Delta_{i-1} } \Pr(j = \piE_k) \Delta_j \Big) \\
        \leq& \sum_{i=1}^A\sum_{k=k_{{i}-1}+1}^{k_{{i}}} \Big(\sum_{\Delta_j \geq \Delta_{i-1}} \big(\frac{2}{k^{2\alpha}} + \frac{2A}{k^{2\alpha-1}}\big) \Delta_j + \sum_{\Delta_j < \Delta_{i-1} } \Pr(j = \piE_k) \Delta_j \Big) \tag{Lemma \ref{lem:combining_UCB_with_LCB_new}}\\
        \leq& \sum_{i=1}^A\sum_{k=k_{{i}-1}+1}^{k_{{i}}} \Big(\sum_{\Delta_j \geq \Delta_{i-1}} \big(\frac{2}{k^{2\alpha}} + \frac{2A}{k^{2\alpha-1}}\big) \Delta_j + \sum_{\Delta_j \leq \Delta_i } \Pr(j = \piE_k) \Delta_j \Big) \tag{$\Delta_i \leq \Delta_{i-1}$}\\
        \leq& \sum_{i=1}^A\sum_{k=k_i+1}^\infty \big(\frac{2}{k^{2\alpha}} + \frac{2A}{k^{2\alpha-1}}\big) + \sum_{i=1}^A\sum_{k=k_{{i}-1}+1}^{k_{{i}}} \sum_{\Delta_j \leq \Delta_i } \Pr(j = \piE_k) \Delta_j \\
        \leq& \sum_{i=1}^A\sum_{k=k_i + 1}^\infty \frac{2(A+1)}{k^{2\alpha-1}}  + \sum_{i=1}^A\sum_{k=k_{{i}-1}+1}^{k_{{i}}} \sum_{\Delta_j \leq \Delta_i } \Delta_i \tag{Second term is maximized when $\Pr(i=\piE_k)=1$.}\\
        \leq& \tilde{O}(\frac{A}{\alpha - 1}) + \sum_{i=1}^A \Delta_i\cdot (k_i - k_{i-1}) \tag{First term: Lemma \ref{lem:integral_lem} and some simplification; Second term: Definition of $k_{i}$.}\\
        =& \tilde{O}(\frac{A}{\alpha - 1}) + \sum_{i:\Delta_i>0} \Delta_i\cdot (k_i - k_{i-1}) \\
        \leq& \tilde{O}(\frac{A}{\alpha - 1}) + \sum_{\Delta_i > 0} 32\alpha c|\Gu_{i-1}|\Big(\frac{1}{\Delta_i}- \frac{\Delta_i}{\Delta_{i-1}^2}\Big)\log(1+\frac{\alpha A}{\Delta_{\min}}) \\
        \approx& \tilde{O}\left(\frac{A}{\alpha - 1} +\sum_{\Delta_i > 0} \alpha |\Gu_{i-1}|\Big(\frac{1}{\Delta_i}- \frac{\Delta_i}{\Delta_{i-1}^2}\Big)\right)
    \end{align*}
    According to the definition, we always have $|\Gu_{i-1}| \leq A - i + 1$, therefore,
    \begin{align*}
        \lim_{K \rightarrow \infty} \Regret_K(\algE) = \tilde{O}\left(\frac{A}{\alpha - 1} +\alpha \sum_{\Delta_i > 0} (A-i)\Big(\frac{1}{\Delta_i}- \frac{\Delta_i}{\Delta_{i-1}^2}\Big)\right)
    \end{align*}
\end{proof}


==> arxiv /Preliminary.tex <==

\section{Preliminary and Problem formulation}\label{sec:learning_framework}
% \subsection{Setting}
\textbf{Stochastic Multi-Armed Bandits (MABs)}~~The MAB model consists of a set of arms $\cA=\{1,2,...,A\}$. When sampling an arm $i\in\cA$, the agent observes a random variable $r_i\in[0,1]$. We use 
$\mu_i = \EE[r_i]$ to denote the mean value for arm $i$ for each $i\in\cA$.
We allow the optimal arms to be non-unique.
For simplicity of notation, we assume the arms are ordered such that $\mu_1 \leq \mu_2...\leq \mu_A$.
% For simplicity of notation, we enumerate the arms according to their expected reward, i.e. $\mu_1 \geq \mu_2 ...\geq \mu_A$. To avoid triviality, we only consider the case when $\mu_1 > \mu_A$, and 

\textbf{Finite-Horizon Tabular Markov Decision Processes (MDPs)}~~For the reinforcement learning (RL) setting, we consider the episodic tabular MDPs denoted by $M(\cS, \cA, H, P, r)$, where $\cS$ is the finite state space, $\cA$ is the finite action space, $H$ is the horizon length, and $\mP=\{\mP_h\}_{h=1}^H$ and $r=\{r_h\}_{h=1}^H$ are the time-dependent transition and reward functions, respectively. 
We assume all steps share the state and action space (i.e. $\cS_1=\cS_2...=\cS_H=\cS$, $\cA_1=\cA_2...=\cA_H=\cA$) while the transition and reward functions can be different.
At the beginning of each episode, the environment will start from a fixed initial state $s_1$ (w.l.o.g.). Then, for each time step $h\in[H]$, the agent selects an action $a_h \in \cA$ based on the current state $s_h$, receives the reward $r_h(s_h,a_h)$, and observes the system transition to the next state $s_{h+1}$, until $s_{H+1}$ is reached. W.l.o.g., we assume the reward function $r$ is deterministic and our results can be easily extended to handle stochastic rewards.

A time-dependent policy is specified as $\pi=\{\pi_1,\pi_2,...,\pi_H\}$ with $\pi_h: \cS\to \Delta(\cA)$ for all $h\in[H]$. Here $\Delta(\cA)$ denotes the probability simplex over the action space.
With a slight abuse of notation, when $\pi_h$ is a deterministic policy, we use $\pi_h:\cS\to \cA$ to refer to a deterministic mapping. $V^\pi_h(s)$ and $Q^\pi_h(s,a)$ denote the value function and Q-function at step $h\in[H]$, which are defined as:
% \begin{align*}
    $
    V^\pi_h(s)=\EE[\sum_{h'=h}^H r_{h'}(s_{h'},a_{h'})|s_h=s,\pi],\quad Q^\pi_h(s,a)=\EE[\sum_{h'=h}^H r_{h'}(s_{h'},a_{h'})|s_h=s,a_h=a,\pi].
    $
% \end{align*}

We use $V^{*}_h(\cdot):=\max_\pi V^\pi_h(\cdot)$ and $Q^{*}_h(\cdot,\cdot)=\max_\pi Q^{\pi}_h(\cdot,\cdot)$ to refer to the optimal state/action-value functions, and  $\Pi^*(s_h):=\{a_h|Q^{*}(s_h,a_h)=V^*_h(s_h)\}$ to denote the collection of all optimal actions at state $s_h$. With an abuse of notation, we define $\Pi^* := \{\pi: V_1^\pi(s_1) = V_1^*(s_1)\}$, i.e., the set of policies that maximize the total expected return. In this paper, when we say that the MDP has ``unique optimal (deterministic) policy'', it is up to the occupancy measure, that is, all policies in $\Pi^*$ share the same state-action occupancy $d^{\pi}(s_h,a_h):=\Pr(S_h=s_h,A_h=a_h|S_1=s_1,\pi)$ for all $h\in[H],s_h\in\cS_h,a_h\in\cA_h$.
%Therefore, we say an MDP has ``unique optimal (deterministic) policy'' if and only if for each state that are reachable by an optimal policy, there is a unique optimal action.
%Besides, if $\pi_1^*\in\Pi^*$ and $\pi_2^*$ only disagrees with $\pi_1^*$ on those states unreachable by $\pi_1^*$, we will not add $\pi_2^*$ into $\Pi^*$.
In the following, we use $|\Pi^*|=1$ to refer to the case of unique optimal (deterministic) policy, where the cardinality of $\Pi^*$ is counted up to the equivalence of occupancies.
Besides, for any function $V:\cS\rightarrow\mR$, we denote $\mP_h V(s_h,a_h) := \EE_{s_{h+1}\sim \mP_h(\cdot|s_h,a_h)}[V(s_{h+1})]$.
% Given a deterministic policy $\pi$, $\pi_h(s_h)\not\in\Pi^*(s_h)$ denotes that $\pi_h$ does not select one of the optimal actions at state $s_h$.
% For simplicity, we use $\cZ_h:=\cS_h\times\cA_h$ to refer to the set of state action pair, and use
% $
% \cZ_{h}^*:=\{(s_h,a_h)| \exists \pi^*\in \Pi^*,~s.t.~d^{\pi^*}(s_h) > 0\}
% $
% to denote the set of states and actions which can be covered by at least one deterministic optimal policy. 
% Our results in this paper also hold for the general case when $|\Pi^*(s_h)| > 1$ for some states, which sometimes implies that there are multiple deterministic optimal policies, i.e. $|\Pi^*| > 1$.

% Since all the optimal policies (both deterministic and stochastic) have the same optimal value function, we will use $V^{*}_h(\cdot)$ and $Q^{*}_h(\cdot,\cdot)$ to refer to the optimal value functions. When there are multiple optimal policies (equivalent to $|\Pi^*|>1$), we may clarify which optimal policy in $\Pi$ we are referring to as $\pi^*$ %in $V^{\pi^*}_h(\cdot)$ and $Q^{\pi^*}_h(\cdot,\cdot)$ 
% whenever necessary.

\textbf{Gap-Dependent Setting}~~We follow the standard formulation of gap-dependent setting in previous bandits \citep{lattimore2020bandit} and RL literature \citep{simchowitz2019non, xu2021fine, dann2021beyond}. 
In bandits, the gap w.r.t.~arm $i$ is defined as $\Delta_i:=\max_{j\in[A]}\mu_j - \mu_i,\forall i \in [A]$, and we assume that there exists a strictly positive value $\Delta_{\min}$ such that, either $\Delta_i = 0$ or $\Delta_i \geq \Delta_{\min}$.
For tabular RL setting, we define $\Delta_h(s_h,a_h):=V^*(s_h)-Q^*(s_h,a_h),\forall h\in[H],s_h\in\cS_h,a_h\in\cA_h$. We use the same notation $\Delta_{\min}$ to refer to the minimal gap in tabular setting and assume that either $\Delta_h(s_h,a_h)=0$ or $\Delta_h(s_h,a_h) \geq \Delta_{\min}$. 

\textbf{Performance Measure}~~We use 
% the learning framework in Framework \ref{alg:general_learning_framework}, and use 
Pseudo-Regret defined below to measure the performance of $\algO$ and $\algE$. 
In the following, we will also use ``exploitation regret'' to refer to $\Regret_K(\algE)$.
\begin{definition}[Pseudo-Regret]\label{def:Pseduo_regret}
We define the regret of $\algO$ and $\algE$ to be:
\begin{align*}
    \Regret_K(\algO):=&\EE\left[\sum_{k=1}^K V_1^*(s_1)-V_1^{\piO_k}(s_1)\right];\quad 
    \Regret_K(\algE):=\EE\left[\sum_{k=1}^K V_1^*(s_1)-V_1^{\piE_k}(s_1)\right],
\end{align*}
where $\piO_k$ and $\piE_k$ are generated according to the procedure in Framework \ref{alg:general_learning_framework} and the expectation is taken over the randomness in data generation and algorithms.
\end{definition}

\section{Lower Bound of $\Regret(\algE)$ without Gap Assumption}\label{sec:Regret_lower_bound_without_gap_assump}
In this section, we show that, 
% without the strictly positive gap assumption on the 
in normal tabular RL setting, for arbitrary algorithm pair $(\algO, \algE)$, even if we do not constrain $\algO$ to be near-optimal, the regret of $\algE$ has the same minimax lower bound as algorithms in online setting. We defer the formal statement and proof to Appendix~\ref{appx:lower_bound_for_general_tabular_MDP}.
% \begin{theorem}[Informal Version of Thm. \ref{thm:Regret_Lower_Bound_of_AlgP}]\label{thm:informal_Regret_Lower_Bound_of_AlgP}
%     There exists a constant $c'$, for arbitrary algorithm pair $(\algO, \algE)$, there always exists a hard tabular MDP $M_{hard}$, such that:
%     \begin{align*}
%         \EE_{(\algO, \algE), M_{hard}}[\sum_{k=1}^K V^* - V^{\piE_k}] \geq c'\sqrt{H^3SAK}
%     \end{align*}
%     where the expectation is taken over the randomness of algorithms and MDP.
% \end{theorem}
\begin{restatable}{theorem}{ThmLBNormalMDP}[Lower Bound for $\algE$ without Gap Assumption]\label{thm:Regret_Lower_Bound_of_AlgP}
    There exist positive constants $c,\epsilon_0, \delta_0$, such that, for arbitrary $S \geq 4, A \geq 2, H \geq 2, K \geq \frac{c}{\epsilon_0^2}H^3SA$, and arbitrary algorithm pair $(\algO, \algE)$, there must exist a hard tabular MDP $M_{hard}$,
    % \begin{align*}
        $
        \EE_{(\algO, \algE), M_{hard}}\left[\sum_{k=1}^K V^* - V^{\piE_k}\right] \geq \delta_0\sqrt{cH^3SAK},
        $
    % \end{align*}
    where the expectation is taken over the randomness of algorithms and MDP.
\end{restatable}
The theorem above is stating that, comparing with the regret lower bound for online algorithms $\tO(\sqrt{H^3SAK})$ in Theorem 9 of \citet{domingues2021episodic}, the exploitation algorithm cannot reduce the dependence on any of parameters $H,S,A,K$ in hard MDPs, even if we allow $\algO$ to sacrifice its performance to gather the best possible data for $\algE$. 
Also, the lower bound would still hold even if we allow both $\algO$ and $\algE$ to additionally use the data $\tauE$ generated by $\piE$.
This negative result implies that without any further assumptions, the separation is not beneficial from a minimax optimality perspective, and we can simply choose both $\algE$ and $\algO$ to be the same near-optimal online algorithm as  without worrying about separating them. %$\algE$ can at best achieve a constant-level improvement comparing with $\algO$ from the minimax optimality perspective, 
%which is not very appealing from a theoretical point of view.

However, in the next section,
% s \ref{sec:analysis_for_MAB} and \ref{sec:Tabular_RL}, 
we will show that, in tabular MDPs with strictly positive gaps, in contrast with the $\Omega(\log K)$ lower bound for online algorithms, we can have $\algE$ such that its regret is constant and independent on the number of time horizon $K$, which reveals the fundamental differences between the pure online setting and the Tiered RL setting considered in this paper.

% \paragraph{Proof sketch of Theorem~\ref{thm:Regret_Lower_Bound_of_AlgP}}
% Our proof is based on the conversion from sublinear regret algorithms to PAC algorithms.
% The main idea is that, given arbitrary algorithm pair $(\algO, \algE)$, we can convert it to a PAC algorithm by uniformly randomly selecting a $\piE_k$ from history and obtain a PAC guarantee from the regret of $\algE$. 
% Combining the lower bound of PAC algorithms \citep{dann2017unifying}, we can infer a lower bound for the regret of $\algE$. 

%Moreover, although in this paper, we focus on Framework \ref{alg:general_learning_framework} and do not consider how to use the data generated by $\piE$, we can use the same techniques in Thm. \ref{thm:Regret_Lower_Bound_of_AlgP} to establish a $O(\sqrt{H^3SAK})$ lower bound even if $\tauE$ are used by $\algE$.
% \blue{From another perspective, our results reflect the tightness of the online to PAC conversion. (whether/how to state this?)}

% The reason why we consider the gap-dependent setting is that, without the gap assumption above, we can prove that no matter what the $\algO$ and $\algE$ are, there always exists a hard MDP such that the regret $\algE$ is $O(\sqrt{H^3SAK})$, which is the same as the minimax lower bound of online algorithms. 
% We defer the details for the lower bound to Sec. \ref{sec:Regret_lower_bound_without_gap_assump}, after we introduce the definition of regret and learning framework in Sec. \ref{sec:learning_framework}.


==> arxiv /Provably_Benefit_in_Stochastic_Bandits.tex <==
\section{Pessimism in the Face of Uncertainty and Constant Regret}\label{sec:PVI_and_ConstantRegret}
In this section, we consider the gap-dependent setting and contribute to identifying the possibility to achieve constant regret by using pessimistic algorithms for $\algE$.
Intuitively, the main reason why PVI can lead to a constant regret is that the quality of the policy returned by PVI is positively correlated to the accumulation of optimal trajectories in the dataset $D$, which is directly connected with $\Regret(\algO)$.
As a result, on the one hand, the regret minimization objective of $\algE$ coincidentally aligns with the optimality constraint of $\algO$.
On the other hand, thanks to the positive gap assumption, $\piE$ will gradually converge to the optimal policy with high probability when $\algE$ is PVI, so there will be no regret after that.
% \wei{The intuition of PVI is very important, but after reading the above intuition twice, I don't feel that I get a good idea out of that.
% 	Isn't that the intuition is more or less as follows: as long as the $\algO$ algorithm performs near optimally, policies (or arms) used in most episodes should be the optimal one, meaning that
% 	the suboptimal policies (arms) are played much less, and this in turn means that the confidence radius of suboptimal policies (arms) would be large and the LCB of the suboptimal policies (arms) would be low.
% 	Therefore, if we use LCB or PVI to select policies (arms) in $\algE$, we are most likely selecting the optimal one.
% 	The above intuitive explanation seems to be good for MAB, but not sure if it is also good for the tabular MDPs. 
% 	In any case, please try to revise the intuition part to be more convincing.
% }
In Sec. \ref{sec:analysis_for_MAB}, we start with stochastic MAB as a warm-up, and in Sec. \ref{sec:Tabular_RL} we extend our success to tabular RL setting. We defer the proofs in this section to Appendix~\ref{appx:analysis_for_bandit_setting}.
\subsection{Warm-Up: Gap-Dependent Regret Bound for Stochastic Multi-Armed Bandits}\label{sec:analysis_for_MAB}

% As discovered by \citep{rouyer2020tsallis}, without the constraint on the performance of $\algO$, $\algE$ can achieve constant regret.
% However, as we briefly mentioned in Sec. \ref{sec:introduction}, the IS estimator in their methods can prevent its extension to RL setting because of the "curse of horizon" problem.
% In contrast, bonus term based exploration and exploitation are provably efficient in RL.
% Therefore, we consider bonus-term based learning framework for $\algE$ based on Pessimistic in the Face of Uncertainty. 
% \red{Moreover, the exploration algorithm in \citep{rouyer2020tsallis} incurs large regret, whereas in our setting we aim
% 	at achieving near-optimal regret for the online algorithm $\algO$ while achieving constant regret for $\algE$.}
 %we introduce our learning framework for $\algE$ based on Pessimistic in the Face of Uncertainty.
% \subsubsection{Algorithm: UCB as $\algO$ and LCB for $\algE$}
\begin{algorithm}
    \textbf{Initilize}: $\alpha > 1;\quad N_i(1) \gets 0,~ \hat\mu_i(1)\gets 0,~\forall i \in \cA;\quad f(k):=1+16A^2(k+1)^2$\\
    \For{$k=1,2,...,K$}{
        % // Choose UCB as $\algO$ and LCB as $\algE$: \\
        $\piO_k \gets \arg\max_i \hat\mu_i(k) + \sqrt{\frac{2\alpha\log f(k)}{N_i(k)}},\quad\quad\piE_k \gets \arg\max_i \hat\mu_i(k) - \sqrt{\frac{2\alpha\log f(k)}{N_i(k)}}.$\\
        Interact with $\groupE$ and $\groupO$ by $\piE_k$ and $\piO_k$, and observe reward $r(\piE_k)$ and $r(\piO_k)$, respectively. \\
        % Pull arm according to $\piE_k$ and observe reward $r(\piE_k)$. \red{env here?}
        % // Note that we do not use this data in learning \\
        \For{$i=1,2,...,A$}{
            $N_{i}(k+1) \gets N_i(k) + \mathbb{I}[\piO_k=i];\qquad \hat{\mu}_i(k+1) \gets \hat{\mu}_i(k)\frac{N_i(k)}{N_i(k+1)}+r(\piO_k)\frac{\mathbb{I}[\piO_k=i]}{{N_i(k+1)}}.$ 
        }
    }
    \caption{UCB-Exploration-LCB-Exploitation}\label{alg:UCB_Explore_LCB_Exploit}
\end{algorithm}
Our main algorithm for bandit setting is shown in Alg \ref{alg:general_learning_framework}, where we consider the UCB algorithm \citep{lattimore2020bandit} as $\algO$ and choose the LCB as $\algE$, which flips the sign of the bonus term in UCB.
We use $N_i(k)$ to denote the number of times that arm $i$ was pulled previous to step $k$, and use $\hat\mu_i$ to record the empirical average of arm $i$. 
Besides, we assume $1/N_i(\cdot)=+\infty$ if $N_i(\cdot)=0$, which implies that at the first $|\cA|$ steps the algorithm will pull each arm one by one.
Moreover, as we will show later, the choice of $\alpha > 1$ is crucial to avoiding dependence on $K$ in $\Regret(\algE)$ with our techniques. 
For Alg. \ref{alg:UCB_Explore_LCB_Exploit}, we have the following guarantee:
% We first state our main theorem about the exploitation regret.
\begin{restatable}{theorem}{ThmLCBRegret}[Exploitation Regret]\label{thm:total_regret_UCB_LCB}
    In Algorithm \ref{alg:UCB_Explore_LCB_Exploit}, by choosing arbitrary $\alpha > 1$, there exists an absolute constant $c$, such that, for arbitrary $K \geq 1$, the pseduo-regret of $\algE$ is upper bounded by:
    % \begin{align*}
        % $
        % \Regret_K(\algE) \leq \sum_{i:\Delta_i > 0} \Big(A\Delta_i + c\cdot \frac{4\alpha A}{\Delta_i}\log(1+\frac{2\alpha A}{\Delta_i})+ \frac{\Delta_i^{4\alpha-4}}{\alpha-1}\Big).
        % $
    % \end{align*}
    % $
    %     \Regret_K(\algE) \leq \frac{A}{\alpha - 1} + \sum_{\Delta_i>0} c\alpha A\cdot \frac{\Delta_i-\Delta_{i+1}}{\Delta_i^2}\log(1+\frac{\alpha A}{\Delta_i}) \approx \tilde{O}(\sum_{\Delta_i > 0} \frac{A(\Delta_i-\Delta_{i+1})}{\Delta_i^2}).
    % $
    $
        \Regret_K(\algE) \leq \tilde{O}\left(\frac{A}{\alpha - 1} +\alpha \sum_{\Delta_i > 0}  (A-i)\Big(\frac{1}{\Delta_i}- \frac{\Delta_i}{\Delta_{i-1}^2}\Big)\right)
    $ 
    % where $\frac{\Delta_i}{\Delta_{i-1}^2} := 0$ when $i=1$. 
    where $\Delta_0 := \infty$ so $\frac{\Delta_1}{\Delta_{0}^2} = 0$.
    % \jiawei{is this formula clear? e.g. will reviewer confused about what is $\Delta_{i-1}$?} \nan{How about ``where the $\Delta_{i}/\Delta_{i-1}^2$ term is $0$ when $i=1$''}.
\end{restatable}
Our result implies that by choosing PVI as $\algE$, we can achieve constant regret while keeping $\algO$ near-optimal.
% As already discussed in Sec. \ref{sec:related_work}, when comparing to \citet{rouyer2020tsallis}, our algorithm can handle non-unique optimal arms and it does not sacrifice the performance of the online algorithm.
Besides the advantages discussed in the related work paragraph in Sec.~\ref{sec:introduction}, our guarantee is also more favorable in certain cases compared to the $O(\sqrt{\frac{A}{\Delta_{\min}}}\sqrt{\sum_{\Delta_i > 0}\frac{1}{\Delta_i}})$ result in \citet{rouyer2020tsallis}: while 
it is not easy to verify whether our guarantee dominates theirs, in many cases ours can be strictly better (or at least no worse) than theirs. For example, consider the following two representative cases: $\Delta_1=\Delta_2=...\Delta_{A-1}=\Delta_{\min}$ (uniform gap) and $\Delta_1=\Delta_2=...=\Delta_{A-2}\gg\Delta_{A-1}=\Delta_{\min}$ (small last gap); our result achieves $\tO(\frac{A}{\Delta_{\min}})$ and $\tO(\frac{1}{\Delta_{\min}})$, respectively, in contrast to their $\tO(\frac{A}{\Delta_{\min}})$ and $\tO(\frac{\sqrt{A}}{\Delta_{\min}})$. 
% \jiawei{I haven't found a simple choice of $\Delta_i$'s when their bound is tighter but it is not easy to prove ours can dominate theirs.
% although our result may have higher dependence on $A$ in some cases, ours can be strictly better than theirs in some other cases.}
% % matches it in some special cases but has higher dependence on $A$ in some other cases. 
% For example, considering the following three cases: (i) $\Delta_1=\Delta_2=...\Delta_{A-1}=\Delta_{\min}$, (ii) $\Delta_1=...=\Delta_{\lceil \sqrt{A} \rceil} = \frac{\Delta_{\min}}{}...\Delta_{A-\lceil\sqrt{A}\rceil}\gg \Delta_{A-\lceil\sqrt{A}\rceil+1}=...=\Delta_{A-1}=\Delta_{\min}$ and (iii) $\Delta_1=\Delta_2=...=\Delta_{A-2}\gg\Delta_{A-1}=\Delta_{\min}$, our result predict $\tO(\frac{A}{\Delta_{\min}})$, $\tO(\frac{\sqrt{A}}{\Delta_{\min}})$ and $\tO(\frac{1}{\Delta_{\min}})$, respectively, in contrast with theirs: $\tO(\frac{A}{\Delta_{\min}})$, $\tO(\frac{\sqrt{A}}{\Delta_{\min}})$ and $\tO(\frac{\sqrt{A}}{\Delta_{\min}})$.
% , which mainly results from our analysis that chooses the average $k/A$ as the benchmark (see Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_A}). 
% It is still an open problem whether the additional $A$ can be improved under the constraint that $\algO$ is near-optimal and we leave it to the future work.

\textbf{Proof Sketch}: The proof consists of two novel technique lemmas with a carefully chosen failure rate $\delta_k \sim O(1/k^{\Theta(\alpha)})$ so that the accumulative failure probability $\sum_{k=1}^\infty\delta_k<+\infty$. 
The first one is Lem. \ref{lem:blessing_of_pessimism}, where we show that w.p.~$1-\delta_k$, LCB will not prefer $i$ with $\Delta_i > 0$ as long as another better arm has been visited enough times in the dataset.
% for arbitrary $i$ with $\Delta_i > 0$, LCB will not prefer $i$ as long as %another event happens that 
% there exists another arm $j$ with $0\leq\Delta_j < \Delta_i$ such that $N_j(k)$ is large enough.
The second step is to identify a key property of UCB algorithm as stated in Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar}, where we provide a high probability upper bound that $N_i(k) \leq k / \lambda$ if $k\geq \tTheta({\lambda}/{\Delta_i^2})$ for arbitrary $\lambda \in [1, 4A]$, and it serves to indicate that the condition required by the success of LCB is achievable as long as $k$ is large enough 
\footnote{Comparing with results in Thm. 8.1 of \citep{lattimore2020bandit}, although our upper bounds of $N_i(k)$ is linear w.r.t. $k$ rather than $\log$ scale, we want to highlight that ours hold with high probability $O(1-k^{-\Theta(\alpha)})$ while \citep{lattimore2020bandit} only upper bounded the expectation.}.
\begin{restatable}{lemma}{LemBlessingLCB}[Blessing of Pessimism]\label{lem:blessing_of_pessimism}
    With the choice that $f(k)=1+16A^2(k+1)^2$, for arbitrary $i$ with $\Delta_i > 0$, for the LCB algorithm in Alg \ref{alg:UCB_Explore_LCB_Exploit}, and arbitrary $j$ satisfying $\Delta_j < \Delta_i$, we have:
    % \begin{align*}
        $
        \Pr\left(\{i = \piE_k\}\cap \{\Delta_j < \Delta_i\} \cap \left\{N_j(k) \geq \frac{8\alpha\log f(k)}{(\Delta_j - \Delta_i)^2}\right\}\right) \leq \frac{2}{k^{2\alpha}}.
        $
    % \end{align*}
\end{restatable} 
\begin{restatable}{lemma}{LemLBofNiNew}[Property of UCB]\label{lem:upper_bound_of_Nk_geq_k_div_scalar}
    With the choice that $f(k)=1+16A^2(k+1)^2$, there exists a constant $c$, for arbitrary $i$ with $\Delta_i > 0$ and arbitrary $\scalar\in[1, 4A]$, in UCB algorithm, we have:
    % \begin{align*}
        $
        \Pr(N_i(k) \geq \frac{k}{\scalar}) \leq \frac{2}{k^{2\alpha-1}},\quad\forall k \geq \scalar + c\cdot\frac{\alpha \scalar}{\Delta_i^2} \log(1+\frac{\alpha A}{\Delta_{\min}}).
        $
    % \end{align*}
\end{restatable}

% \begin{restatable}{lemma}{LemLBofNi}[Property of UCB]\label{lem:upper_bound_of_Nk_geq_k_div_A}
%     With the choice that $f(k)=1+16A^2(k+1)^2$, there exists a constant $c$, for arbitrary $i$ with $\Delta_i > 0$, in UCB algorithm, we have:
%     % \begin{align*}
%         $
%         \Pr(N_i(k) \geq \frac{k}{A}) \leq \frac{2}{k^{2\alpha-1}},\quad\forall k \geq A + c\cdot\frac{\alpha A}{\Delta_i^2} \log(1+\frac{2\alpha A}{\Delta_i}).
%         $
%     % \end{align*}
% \end{restatable}
Directly combining the above two results, we can obtain an upper bound for $\Regret(\algE)$ of order $\tO(A/\Delta_{\min}^{-2})$, which is already independent of $K$.
To achieve better dependence on $\Delta_{\min}$ in the regret, we conduct a finer analysis.
For each arm $i$ with $\Delta_i > 0$, we separate all the arms including $i$ into two groups based on whether its gap exceeds $\Delta_i / 2$: $\Gl_i=\{j:\Delta_j > \Delta_i / 2\}$ and $\Gu_i=\{j:\Delta_j \leq \Delta_i / 2\}$. 
As a result of Lem. \ref{lem:blessing_of_pessimism}, we know that $\piE_k$ will not prefer arm $i$ as long as there exists $j \in \Gu_i$ such that $N_j(k)=\tOmega(4\Delta^{-2}_i)=\tOmega(\Delta_i^{-2})$.
Based on Lem. \ref{lem:upper_bound_of_Nk_geq_k_div_scalar}, we know it is true with high probability, as long as $k \geq \tTheta(A\cdot\Delta_i^{-2})$, since at that time $N_l(k) \leq k / A$ holds for arbitrary $l\in \Gl_i$, which directly implies that $\max_{j:j\in \Gu_i} N_j(k)\geq \tOmega(\Delta_i^{-2})$. Then, combining Lem. \ref{lem:blessing_of_pessimism}, with high probability, the regret resulting from taken arm $i$ cannot be higher than $ \tTheta(A\cdot\Delta_i^{-2}) \cdot \Delta_i = \tTheta(A\cdot\Delta_i^{-1})$, which results in a $\tO(\sum_{\Delta_i > 0} A/\Delta_i)$ regret bound. 
As for the techniques leading to the further improvement in our final result, please refer to Lem. \ref{lem:combining_UCB_with_LCB_new} and the proof of Thm. \ref{thm:total_regret_UCB_LCB} in Appx. \ref{appx:analysis_for_bandit_setting}.

% we 
% can finish the proof by: %we can conclude that:
% \begin{align*}
%     &\Regret_K(\algE):=\sum_{i:\Delta_i > 0}\sum_{k=1}^K \Pr(i=\piE_k)\Delta_i\leq \sum_{i:\Delta_i > 0}\tO(\frac{A}{\Delta_i^2})\cdot \Delta_i + \sum_{k=\tO(\frac{A}{\Delta^2_i})}^K \tO(\frac{A}{k^{2\alpha-1}})\cdot\Delta_i
%     % \leq& \sum_{i:\Delta_i > 0}\tO(\frac{A}{\Delta_i^2})\cdot \Delta_i + \sum_{k=\tO(\frac{A}{\Delta^2_i})}^K \tO(\frac{A}{k^{2\alpha-1}})\cdot\Delta_i 
%     % = \sum_{i:\Delta_i > 0}\tO(\frac{A}{\Delta_i})+\sum_{k=\tO(\frac{A}{\Delta^2_i})}^K \tO(\frac{A}{k^{2\alpha-1}})\cdot\Delta_i.
% \end{align*}
% Therefore, by choosing $\alpha > 1$ such that $\sum 1/k^{2\alpha-1}$ converges to a constant, we can achieve a constant regret bound at level $O(\Delta^{-1}_{\min})$, and complete the proof of Theorem \ref{thm:total_regret_UCB_LCB}. 
% According to the theorem, it is better to consider $\alpha$ slightly larger than 1 (e.g. $\alpha=2$) 
% % because of the term $\frac{\alpha}{\alpha-1}$ coming from the failure rate $\sum^K_k\delta_k$, while
% since larger $\alpha$ may also result in larger regret because it inflates the bonus term and slows down the identification of the optimal arm.

% Finally, as a result of the amplification factor $\alpha$ in Algorithm \ref{alg:UCB_Explore_LCB_Exploit}, the failure rate $\delta_k$ above can be controlled by $O(k^{-2\alpha+1})$ (or maybe $O(k^{-2\alpha})$). Therefore, by choosing $\alpha$ appropriately, we can control the regret when the ``good events'' are violated by relating it with the sum of a converged sequence $1/k^{-2\alpha+1}$: $\sum_{k=1}^\infty \delta_k \Delta_i \leq \sum_{k=1}^\infty k^{-2\alpha+1}\Delta_i < c\Delta_i < \infty$ for some constant related to the choice of $\alpha$. As a result, we can provide an upper bound for the expected regret without dependence on the episodes $K$.

% We first define a threshold $k_{f,A,\alpha,\Delta_{\min}}:=2A+c_{f,A,\alpha,\Delta_{\min}} \frac{\alpha A}{\Delta_{\min}^2}\log(A+\frac{\alpha A}{\Delta_{\min}})$, where $c_{f,A,\alpha,\Delta_{\min}}$ is a constant, and use it to separate the regret analysis into two parts: the accumulative regret from step $k=1$ till $k=k_{f,A,\alpha,\Delta_{\min}}$ and the regret after $k=k_{f,A,\alpha,\Delta_{\min}}$. Concretely, the decomposition is:
% \begin{align*}
%     \EE[\Regret(\algE)] \leq & \sum_{i:\Delta_i > 0} \Big(P(N_i(k_{f,A,\alpha,\Delta_{\min}}) \leq \tilde{N}_i) \cdot \tilde{N}_i \cdot \Delta_i + P(N_i(k_{f,A,\alpha,\Delta_{\min}}) \geq \tilde{N}_i)\cdot k_{f,A,\alpha,\Delta_{\min}} \cdot \Delta_i\Big) \\
%     &\quad\quad+ \sum_{i:\Delta_i > 0} \sum_{k=k_{f,A,\alpha,\Delta_{\min}}+1}^\infty P(\piE_k=i)\Delta_i
% \end{align*}
% where $\tilde{N}_i$ is a carefully choosen threshold, to trade-off between the magnititude of $\tilde{N}_i$, and $P(N_i(k_{f,A,\alpha,\Delta_{\min}})\geq \tilde{N}_i)$, which correspond to the magnititude of the first and the second term, respectively. 

% For the last term, we leverage the advantage of the Pessimism. Because of the \red{"double gaurantee" property} of LCB, by proving an additional lemma and providing a lower bound of $N_{i^*}(k)$, we can show that $P(\piE_k=i)$ can be upper bounded by a converged series $1/k^O(\alpha)$, and therefore, we a propoer choice of $\alpha$, it is also be controlled at the constant level.

% \blue{the choice of $k_{f,A,\alpha,\Delta_{\min}}$ trade-offs three parts...}

==> arxiv /Provably_Benefit_in_Tabular_MDP.tex <==
\subsection{Constant Regret of $\algE$ in Tabular MDPs}\label{sec:Tabular_RL}

% When the optimal policy is unique in the tabular MDP, we show that the regret of $\algE$ is also constant and only depends on $O(\text{Poly}(S,A,H,\frac{1}{\Delta_{\min}},\log d_{\min}))$. Here $d_{\min}$ is the minimal occupancy of the states reachable by the unique optimal policy $\pi^*$, and we show that it is unavoidable by proving a lower bound.
% \footnote{High-level speaking, it is because we treat $\algO$ as a black box and only leverage its near-optimal regret property. This improves the generality of our results while reducing the constraint on the behavior of $\algO$. We conjecture it is possible to study a concrete choice of $\algO$ to avoid $\log d_{\min}$, and leave it to future work.}.

%  coverage of dataset on optimal policies.
% and possibly result in extremely dispersion of the coverage of dataset to multiple optimal policies instead, 
% especially when the number of optimal policies is exponentially large.


% \subsection{Tiered RL Algorithm for Tabular MDP}
% \begin{algorithm}[H]
%     $D_1\gets \{\}$\\
%     \For{$k=1,2,...,K,...$}{
%         \blue{// Compute $\piO_k$ by $\algO$} \\
%         $\piO_k\gets \algO(D_k,k)$\\
%         \blue{// Compute $\piE_k$ by Pessimistic Value Iteration }\\
%         \For{$h = H,H-1,...,1$}{
%             \For{$s_h \in \cS_h ,a_h \in \cA_h$}{
%                     \begin{align*}
%                     \hmP_h(\cdot|s_h,a_h)\gets 
%                     \begin{cases}
%                         0,\quad & \text{if } N_h(s_h,a_h)=0\\
%                         \frac{N_h(s_h,a_h,\cdot)}{N_h(s_h,a_h)},\quad & \text{otherwise}
%                     \end{cases}
%                     \end{align*}
%                 }
%             $b_h(\cdot,\cdot)\gets \textbf{Bonus}(D, k)$ \\
%             $\hQ_{h}(\cdot,\cdot) \gets \max\{R(\cdot,\cdot)+\hmP_h\hV_{h+1}(\cdot,\cdot) - b_h(\cdot,\cdot), 0\},\quad \hV_h(\cdot) = \max_{a_h\in\cA}\hQ_h(\cdot, a_h)$ \\
%             $\piE_{k,h}(\cdot)\gets \argmax_{a} \hQ_h(\cdot,a)$
%         }
%         Sample one trajectories $\tauO_k:=\{s_{k,1},a_{k,1},...,s_{k,H},a_{k,H}\}\sim \piO_k$.\\
%         $D_{k+1} \gets D_k \cup \{\tauO_k\}$.
%     }    
%     \caption{Tiered RL Algorithm for Tabular MDP}\label{alg:tiered_RL_tabular_MDP}
% \end{algorithm}

In this section, we establish constant regret of $\algE$ based on realistic conditions for $\algO$ and $\algE$. 
We highlight the key steps of our analysis and our technical contributions here.

% Our analysis consists of three parts. 
First of all, in Sec.\ref{sec:PVI_and_Property}, we propose the concrete PVI algorithm, and inspired by the clipping trick used for optimistic online algorithms \citep{simchowitz2019non}, we develop a high-probability gap-dependent upper bound for the sub-optimality of $\piE$, which is related to the accumulation of the optimal trajectories in dataset $D_k$.
Secondly, in Sec. \ref{sec:choice_algO}, we first introduce a general condition (Cond. \ref{cond:requirement_on_algO}) for the chocie of $\algO$,
% arbitrary algorithms satisfying it can be used as $\algO$ in our framework. 
based on which we quantify the accumulation of optimal trajectories in $D_k$ with the regret of $\algO$, and connect the exploration by $\algO$ and the optimality of $\algE$. We also supplement some details about how to relax such a condition and inherit the guarantees by the doubling-trick in Appx. \ref{appx:Doubling_Trick}, which may be of independent interest.
In Sec. \ref{sec:tabular_RL_main_analysis}, i.e. the last part of analysis, we bring the above two steps together and complete the proof. 
However, there is an additional challenge when the tabular MDP has multiple deterministic optimal policies, which is possible when there are non-unique optimal actions at some states. 
We overcome this difficulty by Thm.~\ref{thm:existence_of_well_covered_optpi} about policy coverage. 
To our knowledge, the only paper that runs into a similar challenge is \citep{papini2021reinforcement}, and they bypass the difficulty by assuming the uniqueness of optimal policy. Finally, Section \ref{sec:tabular_RL_Discussion} provide  some interpretation and implications of our results.

% Finally, in Appendix~\ref{appx:Doubling_Trick}, we propose another framework inspired by doubling-trick to extend our achieved results for a more general class of $\algO$, which may be of independent interest.


% In Section \ref{sec:choice_algP}, we introduce the PVI algorithm and its property. In Section \ref{sec:choice_algO}, we introduce a general condition for the online algorithm, and our later guarantee for $\algE$ will apply as long as $\algO$ satisfies the said condition. 
% %. and its implication for the candidates of $\algO$.
% % We also briefly mention the gap between the condition for $\algO$ we establish our analysis on and the existing near-optimal online learning algorithms, and in Appx. \ref{appx:Doubling_Trick} we will close this gap by proposing another extended learning framework based on doubling-trick.
% After that, in Section \ref{sec:tabular_RL_main_analysis}, we present the main result (Thm.~\ref{thm:UB_Regret_PVI}) which is a constant regret guarantee for $\algE$ under the introduced conditions. 

% In this section, we separately consider the cases when the optimal policies are non-unique or not because of the additional technical challenges in non-unique optimal policies setting.

% , the analysis becomes more challenging because $\algO$ may not converge to one particular optimal policy, which causes difficulty for PVI as it needs the data to provide sufficient coverage for at least one optimal policy.

% \blue{
%     \paragraph{\blue{Intuition about why PFU is preferred}}
%     PFU has some interesting property. Intuitively, the performance of PFU based algorithm depends on the number of optimal trajectories and do not be bothered by whether other sub-optimal states and actions are explored enough. That's because, either sub-optimal regions are explored enough or not, as long as the occupancy of optimal trajectories is high enough, PFU algorithm can identify the optimal policy. (For sub-optimal regions, if not explored enough, then it has high uncerntainty; if explored enoughm then we still take optimal policy).
    
%     Thanks to PFU, the success of $\algE$ also relies on the occupancy of optimal trajectories in the dataset generated by policies computed by $\algO$. In this way, $\algE$ will benefit from the success of $\algO$, and in this way, $\algO$ does not have to sacrifice something for $\algE$. 
% }
\subsubsection{Pessimistic Value Iteration as $\algE$ and its Property}\label{sec:PVI_and_Property}
% \subsubsection{Choice and Analysis of $\algE$: Pessimistic Value Iteration}\label{sec:choice_algP}
% \begin{remark}
%     Because the bonus term is always non-negative, we directly have $\hQ_h \leq H-h+1$ because $r \in [0,1]$.
% \end{remark}

% \begin{algorithm}
%     \textbf{Input}: Iteration number $k$; Dataset $D_k$; Confidence level $\delta_k$; Bonus function $\textbf{Bonus}(\cdot,\cdot)$\\
%     \For{$h = H,H-1,...,1$}{
%         \For{$s_h \in \cS_h ,a_h \in \cA_h$}{
%             $N_{k,h}(s_h,a_h)\gets$ the number of times $s_h,a_h$ occurs in the dataset $D_k$.\\
%             $N_{k,h}(s_h,a_h,s_{h+1})\gets$ the number of times $(s_h,a_h,s_{h+1})$ occurs in the dataset $D_k$.\\
%             $
%             \hmP_{k,h}(\cdot|s_h,a_h)\gets 
%             \begin{cases}
%                 0,\quad & \text{if } N_{k,h}(s_h,a_h)=0;\\
%                 \frac{N_{k,h}(s_h,a_h,\cdot)}{N_{k,h}(s_h,a_h)},\quad & \text{otherwise}.
%             \end{cases}
%             $\\
%             }
%         $b_{k,h}(\cdot,\cdot)\gets \textbf{Bonus}(D_k, \delta_k).$ \\
%         $\hQ_{k,h}(\cdot,\cdot) \gets \max\{R(\cdot,\cdot)+\hmP_{k,h}\hV_{k,h+1}(\cdot,\cdot) - b_{k,h}(\cdot,\cdot), 0\},\quad \hV_{k,h}(\cdot) = \max_{a_h\in\cA}\hQ_{k,h}(\cdot, a_h).$ \\
%         $\piPVI_{k,h}(\cdot)\gets \argmax_{a} \hQ_{k,h}(\cdot,a).$
%     }
%     \Return $\piPVI_{k}$.
%     % Sample one trajectories $\tauO_k:=\{s_{k,1},a_{k,1},...,s_{k,H},a_{k,H}\}\sim \piO_k$.\\
%     % $D_{k+1} \gets D_k \cup \{\tauO_k\}$.
%     \caption{Pessimistic Value Iteration}\label{alg:PVI}
% \end{algorithm}

\begin{algorithm}
    \textbf{Input}: Episode number $K$; Confidence level $\{\delta_k\}_{k=1}^K$; Bonus function $\textbf{Bonus}(\cdot,\cdot)$\\
    \For{$k=1,2,...,K$}{
        % // \blue{Run PVI as $\algE$} //
        % // \blue{\textbf{Step 1}: use PVI to compute $\piE_k$ for $\groupE$} \\
        $\{b_{k,1}(\cdot,\cdot), b_{k,2}(\cdot,\cdot), ...,b_{k,H}(\cdot,\cdot)\}\gets \textbf{Bonus}(D_k, \delta_k).$ //\blue{Compute bonus function for PVI.}\\
        \For{$h = H,H-1,...,1$}{ 
            \For{$s_h \in \cS_h ,a_h \in \cA_h$}{
                $N_{k,h}(s_h,a_h)\gets$ the number of times $s_h,a_h$ occurs in the dataset $D_k$.\\
                $N_{k,h}(s_h,a_h,s_{h+1})\gets$ the number of times $(s_h,a_h,s_{h+1})$ occurs in the dataset $D_k$.\\
                $
                \hmP_{k,h}(\cdot|s_h,a_h)\gets 
                \begin{cases}
                    0,\quad & \text{if } N_{k,h}(s_h,a_h)=0;\\
                    \frac{N_{k,h}(s_h,a_h,\cdot)}{N_{k,h}(s_h,a_h)},\quad & \text{otherwise}.
                \end{cases}
                $\\
                }
            $\hQ_{k,h}(\cdot,\cdot) \gets \max\{R(\cdot,\cdot)+\hmP_{k,h}\hV_{k,h+1}(\cdot,\cdot) - b_{k,h}(\cdot,\cdot), 0\}.$ \\
            $\hV_{k,h}(\cdot) = \max_{a_h\in\cA}\hQ_{k,h}(\cdot, a_h),\quad \piPVI_{k,h}(\cdot)\gets \argmax_{a} \hQ_{k,h}(\cdot,a).$
        }
        $\piE_k \gets \{\piPVI_{k,1}, \piPVI_{k,2},...\piPVI_{k,H}\}$ \\
        // \blue{\textbf{Step 2}: Use $\algO$ satisfying Cond. \ref{cond:requirement_on_algO} to compute $\piO_k$ for $\groupO$} \\
        $\piO_k \gets \algO(D_k).$\\
        // \blue{\textbf{Step 3}: Sample trajectories and collect new data} \\
        Interact with $\groupE$ and $\groupO$ by $\piE_k$ and $\piO_k$, and observe $\tauE_k$ and $\tauO_k$, respectively. \\
        $D_{k+1} \gets D_k \cup \{\tauO_k\}$. 
        % // \blue{For convenience, we only consider use data collected by $\piO$.}
    }
    % \Return $\piPVI_{k}$.
    % Sample one trajectories $\tauO_k:=\{s_{k,1},a_{k,1},...,s_{k,H},a_{k,H}\}\sim \piO_k$.\\
    % $D_{k+1} \gets D_k \cup \{\tauO_k\}$.
    \caption{Tiered-RL Algorithm with Pessimistic Value Iteration as $\algE$}\label{alg:PVI}
\end{algorithm}
The full details of our algorithm for tiered RL setting is provided in Alg. \ref{alg:PVI}, where we use PVI as $\algE$. 
Here we do not specify a concrete \textbf{Bonus} function, but provide general results for a range of qualified bonus functions satisfying Cond. \ref{cond:bonus_term} below. Cond. \ref{cond:bonus_term} can be satisfied by many bonus term considered in online literatures, and we briefly dicuss some examples in Appx.~\ref{appx:choice_of_bonus_term}.
% different choice of bonus term will lead to different $B_1$ and $B_2$. 
% We defer the concrete examples to Appendix~\ref{appx:analysis_of_PVI}.

% \begin{condition}[Condition on Bonus Term for $\algE$]\label{cond:bonus_term}
%     For arbitrary confidence level sequence $\{\delta_k\}_{k=1}^K$ with $\delta_k\in (0,1/2)~\forall k\in[K]$, at arbitrary iteration $k\in[K]$ in Alg. \ref{alg:PVI}, the function $\textbf{Bonus}(\cdot,\cdot)$ takes into the dataset $D_k$ and confidence level $\delta_k$ as input, and returns a bonus function $b=\{b_1(\cdot,\cdot),...,b_H(\cdot,\cdot)\}$ where $b_h:\cS\times\cA\rightarrow \mR$. For the event $\cEB$ defined below, the bonus function satisfies $\Pr(\cEB)\geq 1-\delta$ \red{for arbitrary $V$}.
%     \begin{align*}
%         \cEB := \bigcap_{\substack{h\in[H],\\ s_h\in\cS_h,a_h\in\cA_h}}\Big\{\{|\hat \mP_h V_{h+1}(s_h,a_h) - \mP_hV_{h+1}(s_h,a_h)| < b_h(s_h,a_h)\} \cap \{b_h(s_h,a_h) \leq B_1\sqrt{\frac{\log (B_2/\delta)}{N(s_h,a_h)}}\}\Big\}
%     \end{align*}
%     where $\hat \mP_h$ and $V_h$ are computed by running Alg. \ref{alg:PVI} with $D$, and $B_1$ and $B_2$ are parameters depending on $S,A,H$ and gap $\Delta$ but independent of $\delta$. 
%     % Moreover, $\forall h\in[H],s_h\in\cS_h, a_h\in\cA_h$, we have $b_h(s_h,a_h) \leq B_1\sqrt{\frac{\log (B_2/\delta)}{N(s_h,a_h)}}$, where $B_1$ and $B_2$ are parameters depending on $S,A,H$ and gap $\Delta$ but independent of $\delta$.
% \end{condition}

\begin{condition}[Condition on Bonus Term for $\algE$]\label{cond:bonus_term}
    % the function $\textbf{Bonus}(\cdot,\cdot)$ takes into the dataset $D_k$ and confidence level $\delta_k$ as input, and returns a 
    % the bonus functions $\{b_{k,1}(\cdot,\cdot),...,b_{k,H}(\cdot,\cdot)\}$ returned by $\textbf{Bonus}(D_k, \delta_k)$ satisfying the following:
    %  where $b_h:\cS\times\cA\rightarrow \mR$. 
    % For the event $\cEB$ defined below, the bonus function satisfies $\Pr(\cEB)\geq 1-\delta$ \red{for arbitrary $V$}.
    We define the following event at iteration $k\in[K]$ during the running of Alg. \ref{alg:PVI}:
    % \begin{align*}
        % $
        % \cEBk := \bigcap_{\substack{h\in[H],\\ s_h\in\cS_h,\\a_h\in\cA_h}}\Big\{\{|\hat \mP_{k,h} \hV_{k,h+1}(s_h,a_h) - \mP_h\hV_{k,h+1}(s_h,a_h)| < b_{k,h}(s_h,a_h)\} \cap \{b_{k,h}(s_h,a_h) \leq B_1\sqrt{\frac{\log (B_2/\delta_k)}{N_{k,h}(s_h,a_h)}}\}\Big\}
        % $
        $
        \cEBk := \bigcap_{\substack{h\in[H],s_h\in\cS_h,a_h\in\cA_h}}\Big\{\{|\hat \mP_{k,h} \hV_{k,h+1}(s_h,a_h) - \mP_h\hV_{k,h+1}(s_h,a_h)| < b_{k,h}(s_h,a_h)\} \cap \{b_{k,h}(s_h,a_h) \leq B_1\sqrt{\frac{\log (B_2/\delta_k)}{N_{k,h}(s_h,a_h)}}\}\Big\}
        $
    % \end{align*}
    % where $\hat \mP_h$ and $V_h$ are computed by running Alg. \ref{alg:PVI} with $D$, and 
    where $B_1$ and $B_2$ are parameters depending on $S,A,H$ and $\Delta$ but independent of $\delta_k$, $k$.\footnote{Note that 
    % this is just requirement for the upper bound of $b_{k,h}$ while 
    we do not require the knowledge of $\Delta_i$'s to compute $b_{k,h}$.} We assume that, \textbf{Bonus} function satisfies that, in Alg. \ref{alg:PVI}, given arbitrary sequence $\{\delta_k\}_{k=1}^K$ with $\delta_1,\delta_2,...,\delta_K\in (0,1/2)$, at arbitrary iteration $k\in[K]$, we have $\Pr(\cEBk)\geq 1-\delta_k$.
    % Moreover, $\forall h\in[H],s_h\in\cS_h, a_h\in\cA_h$, we have $b_h(s_h,a_h) \leq B_1\sqrt{\frac{\log (B_2/\delta)}{N(s_h,a_h)}}$, where $B_1$ and $B_2$ are parameters depending on $S,A,H$ and gap $\Delta$ but independent of $\delta$.
\end{condition}
Next, we provide an upper bound for the sub-optimality gap of $\piPVI_k$ with the clipping operator $\Clip[x|\epsilon]:=x\cdot \mathbb{I}[x\geq \epsilon]$.
Previous upper bounds of PVI \citep[e.g.,~Theorem 4.4 of][]{jin2021pessimism} do not leverage the strictly positive gap and can be much looser when $N_{k,h}$ is large, and directly applying those results to our analysis would result in a regret scaling with $\sqrt{K}$.
% Based on the clipping trick and the gap assumption, we provide a tighter bound .
% \footnote{One may observe that, in Thm. \ref{thm:clipping_trick}, the clipping threshold $\epsClip'$ for the case (ii) is much smaller than $\epsClip$ for unique optimal policy setting. In fact, when $\pi^*$ is chosen to be some particular optimal policies, one can replace $\epsClip'$ with $\epsClip$ in the upper bound for case (ii). However, the main challenge is that it's not easy to guarantee that those particular choices of $\pi^*$ are well-covered by the dataset (i.e. $N_{k,h}(s_h,a_h)$ is large enough for those $(s_h,a_h)$ reachable by $\pi^*$), because we treat $\algO$ as a black box satisfying Cond. \ref{cond:requirement_on_algO} (as we will introduce later) and its behavior is unpredictable.
% It might be possible to analyze the behavior of some more concrete choices of $\algO$ and establish a much tighter bound than ours, and we leave it for the future work.
% (\red{Question: Here I what to address the concerns about the huge gap between two clipping threshold here, shall we discuss more details in the appendix about what's the regret upper bound with $\epsClip$ as clipping threshold looks like for case (ii)?})
% }
\begin{restatable}{theorem}{ThmClipTrick}\label{thm:clipping_trick}
    By running Algorithm \ref{alg:PVI} with confidence level $\delta_k$, a function \textbf{Bonus} satisfying Condition \ref{cond:bonus_term}, and a dataset $D=\{\tau_1,...\tau_k\}$ consisting of $k$ complete trajectories generated by executing a sequence of policies $\pi_1,...,\pi_k$, on the event $\cEB$ defined in Condition \ref{cond:bonus_term}:
    \begin{align}
        V^{*}_1(s_1)-V_1^{\piPVI_k}(s_1) \leq 
        % 2\EE_{\pi^*}[\sum_{h=1}^H \ddot{\surplus}_{k,h}(s_h,a_h)] = 
        % 2\EE_{\pi^*}[\sum_{h=1}^H \Clip[\surplus_{k,h}(s_h,a_h)|\epsClip]]
        2\EE_{\pi^*}\left[\sum_{h=1}^H \Clip\left[\left. \min \left\{ H, 2B_1\sqrt{\frac{\log (B_2/\delta_k)}{N_{k,h}(s_h,a_h)}} \right\}\right|\epsClip \right] \right].
        \label{eq:sub_opt_clip_case1}
    \end{align}
    % (i) when $|\Pi^*|=1$ (unique optimal deterministic policy) 
    % \begin{align}
    %     V^{*}_1(s_1)-V_1^{\piPVI_k}(s_1) \leq 
    %     % 2\EE_{\pi^*}[\sum_{h=1}^H \ddot{\surplus}_{k,h}(s_h,a_h)] = 
    %     % 2\EE_{\pi^*}[\sum_{h=1}^H \Clip[\surplus_{k,h}(s_h,a_h)|\epsClip]]
    %     2\EE_{\pi^*}\left[\sum_{h=1}^H \Clip\left[\left. \min \left\{ H, 2B_1\sqrt{\frac{\log (B_2/\delta_k)}{N_{k,h}(s_h,a_h)}} \right\}\right|\epsClip \right] \right].
    %     \label{eq:sub_opt_clip_case1}
    % \end{align}
    % \indent (ii) when $|\Pi^*|>1$ (non-unique optimal deterministic policies)
    % \begin{align}
    %     V^*_1(s_1) - V^{\piPVI_k}_1(s_1) \leq
    %     % & 2 \EE_{\pi^*}[\sum_{h=1}^H \Clip[\surplus_{k,h}(s_h,a_h)|\epsClip']]
    %     2\EE_{\pi^*}\left[\sum_{h=1}^H \Clip\left[\left. \min \left\{H, 2B_1\sqrt{\frac{\log (B_2/\delta_k)}{N_{k,h}(s_h,a_h)}} \right\} \right|\epsClip'\right] \right].
    %     \label{eq:sub_opt_clip_case2}
    % \end{align}
    where $\pi^*$ 
    can be an arbitrary optimal policy, $\epsClip:= \frac{\Delta_{\min}}{2H+2}$ if $|\Pi^*|=1$ and $\epsClip:=\frac{d_{\min}\Delta_{\min}}{2SAH}$ if $|\Pi^*|>1$, where $d_{\min}:= \min_{\pi\in\Pi^*,h\in[H],s_h\in\cS_h,a_h\in\cA_h} d^{\pi}(s_h,a_h)$ subject to $d^{\pi}(s_h,a_h) > 0$.
    % (stochastic or deterministic) 
\end{restatable}
% In the theorem above, we define $d_{\min}$ to be:
% \begin{align*}
%     d_{\min}:= \min_{\pi^*\in\Pi^*,h\in[H],s_h\in\cS_h,a_h\in\cA_h} d^{\pi^*}(s_h,a_h),\quad s.t.~d^{\pi^*}(s_h,a_h) > 0.
% \end{align*}
\subsubsection{Choice and Analysis of $\algO$}\label{sec:choice_algO}
% Considering that the behavior of online RL algorithms in tabular RL is more obscure than UCB in MABs, and also for the generality of our results, we analyze the regret of $\algE$  for any $\algO$ that satisfies a general condition given below, 
Next, we introduce our general condition for $\algO$ that the $\algO$ can achieve $O(\log k)$-regret with high probability. 
It is worth noting that many existing near-optimal online RL algorithms for gap-dependent settings may not directly satisfy the condition \citep{simchowitz2019non,xu2021fine,dann2021beyond} since they use a fixed confidence interval $\delta$.
In Appx.~\ref{appx:Doubling_Trick}, we will introduce a more realistic abstraction of those algorithms in Cond.~\ref{cond:realistic_requirement_on_algO}, and discuss in more details about how to close this gap with an algorithm framework inspired by the doubling trick. 
\begin{condition}[Condition on $\algO$]\label{cond:requirement_on_algO}
    $\algO$ is an algorithm which
    % is an ``anytime'' algorithm (i.e. do not require the knowledge of total number of steps), which only 
    returns deterministic policies at each iteration, and for arbitrary $\nk\geq 2$, we have:
    % \begin{align*}
        $
        \Pr\big(\sum_{\tk=1}^\nk V^*_1(s_1)-V^{\piO_\tk}_1(s_1) > C_1 + \alpha C_2 \log \nk \big) \leq \frac{1}{\nk^\alpha},
        $
    % \end{align*}
    where $C_1,C_2$ are parameters only depending on $S,A,H$ and gap $\Delta$ and independent of $\nk$.
\end{condition}
% In Appx. \ref{appx:Doubling_Trick}, we will propose another algorithm framework inspired by the ``Doubling Trick'' and discuss how to generalize our results based on Cond. \ref{cond:requirement_on_algO} to algorithms satisfying Cond. \ref{cond:realistic_requirement_on_algO} instead.
\textbf{Implication of Condition~\ref{cond:requirement_on_algO} for $\algO$}
% An important message implied by Thm. \ref{thm:sub_opt_with_clipping_trick} is that, the more optimal trajectories in the dataset, the smaller the sub-opt gap of $\piE_k$ (or say one-step regret of $\algE$) will be. 
% Actually, this important property makes it possible to achieve the minimization of regret of $\algO$ and lower regret of $\algE$ at the same time, because intuitively, the lower the regret of $\algO$ is, the more chances that $\piO_k$ is optimal will be, which will result in higher frequency of optimal trajectories in the dataset used by $\algE$. 
Intuitively, low regret implies high accumulation of optimal trajectories in the dataset collected by $\algO$. We formalize this intuition in Thm.~\ref{thm:algO_regret_vs_algP_density} by establishing the relationship between the regret of $\algO$, $d^{\pi^*}$ and $\sum_{\tk=1}^k d^{\piO_\tk}(s_h,a_h)$ (the expectation of $N_{k,h}$).
\begin{restatable}{theorem}{ThmORegretPDensity}\label{thm:algO_regret_vs_algP_density}
    For an arbitrary sequence of deterministic policies $\pi_1,\pi_2,...,\pi_k$, there must exist a sequence of deterministic optimal policies $\pi_1^*, \pi_2^*,...,\pi_k^*$, such that $\forall h\in[H], s_h \in\cS_h, a_h\in\cA_h$:
    \begin{align*}
        \sum_{\tk=1}^k d^{\pi_\tk}(s_h,a_h) \geq \sum_{\tk=1}^k d^{\pi^*_\tk}(s_h,a_h) - \frac{1}{\Delta_{\min}} \Big(\sum_{\tk=1}^k V^*_1(s_1)-V^{\pi_\tk}_1(s_1)\Big).
    \end{align*}
\end{restatable}

\subsubsection{Main Results and Analysis}\label{sec:tabular_RL_main_analysis}
The main analysis is based on our discussion about the properties of $\algE$ and $\algO$ in previous sub-sections. 
In the following, we first discuss the proof sketch for the case when $|\Pi^*|=1$.
The main idea is to show that the unique $\pi^*$ will be ``well-covered'' by dataset, where we say a policy $\pi^*$ is ``well-covered'' if for each $(s_h,a_h)\in\cS_h\times\cA_h$ with $d^{\pi^*}(s_h,a_h) > 0$, 
% $N_{k,h}(s_h,a_h)\sim \sum_{\tk=1}^k d^{\pi^*_\tk}(s_h,a_h)$ 
$N_{k,h}(s_h,a_h)$ can strictly increase so that the RHS of Eq.\eqref{eq:sub_opt_clip_case1} in Thm.~\ref{thm:clipping_trick} will gradually decay to zero (e.g. $N_{k,h}(s_h,a_h)\geq \tilde{O}(k)$).
To show this, the key observation is that, 
% for each $(s_h,a_h)$ with $d^{\pi^*}(s_h,a_h) > 0$, 
with high probability, $N_{k,h}(s_h,a_h)$ will not deviate too much from its expectation $\sum_\tk d^{\pi_\tk}(s_h,a_h)$ (Lem. \ref{lem:concentration}), and can be lower bounded by $\sum_{\tk=1}^k d^{\pi_\tk^*}(s_h,a_h)-O(\log k)=kd^{\pi^*}(s_h,a_h)-O(\log k)$ as a result of Thm.~\ref{thm:algO_regret_vs_algP_density}.
% In addition with Lem. \ref{lem:concentration}, with high probability, $N_{k,h}(s_h,a_h) \geq O(kd^{\pi^*}(s_h,a_h)-\log k)$. 
As a result, the clipping operator in Eq.\eqref{eq:sub_opt_clip_case1} will take effects as long as $k$ is large enough, and $\piPVI_k$ will converge to the optimal policy with no regret. 
All that remains is to show the regret under failure events is also at the constant level because we choose a gradually decreasing failure rate $O(\frac{1}{k^\alpha})$, and $\lim_{K\rightarrow \infty}\sum_{k=1}^K O(\frac{1}{k^\alpha})<\infty$ as long as $\alpha > 1$. 
% \red{shall we provide results for high probability results first?}

However, when $|\Pi^*| > 1$, the analysis becomes more challenging.
% Although the $\pi^*$ in Thm. \ref{thm:clipping_trick} can be arbitrary, 
% \blue{Intuitively, since $\algO$ has near-optimal regret, the sub-optimality of $\piE$ will continuously decay till lower than the minimal gap, after which $\algE$ will suffer no more regret.}
% The main reason is that it is not easy to claim that at least one optimal policy is ``well-covered'' by $D_k$ to apply Thm. \ref{thm:clipping_trick}, especially when the number of deterministic optimal policies is very large.
% In order to use Thm.~\ref{thm:clipping_trick} to upper bound $\Regret(\algE)$, we need to show there exists an optimal policy $\pi^*$ (possibly stochastic) ``well-covered'' by the sequence $\pi^*_1,...,\pi^*_k$ in Thm.~\ref{thm:algO_regret_vs_algP_density}, where ``well-covered'' means that for each $(s_h,a_h)\in\cS_h\times\cA_h$ with $d^{\pi^*}(s_h,a_h) > 0$, $N_{k,h}(s_h,a_h)\sim \sum_{\tk=1}^k d^{\pi^*_\tk}(s_h,a_h)$ increases strictly faster than $\log k$, 
% is strictly increasing w.r.t.~$k$ 
% the value inside the clipping operator will gradually decay to threshold with high probability.
The main difficulty is that, when the optimal policy is not unique,
% Although Thm.~\ref{thm:clipping_trick} can be applied to arbitrary optimal policy $\pi^*$, because of $|\Pi^*|>1$, 
it is not obvious about the existence of ``well-covered'' $\pi^*$, since it is not guarantee that how much similarity is shared by the sequence of policies $\pi_1^*,...\pi^*_k$, especially when $|\Pi^*|$ is exponentially large (e.g. $|\Pi^*|=\Omega((SA)^H)$).
% there exists a policy $\pi^*$ that occurs in the policy sequence $\pi^*_1,...,\pi^*_k$ for $O(k)$ times, and choosing $\pi^*$ to be the mixture policy $\pi_{mix}:=\frac{1}{k}\sum_{\tk=1}^k \pi^*_k$ also does not work since it's possible that $d^{\pi_{mix}}(s_h,a_h)=O(\frac{1}{k})$ if $a_h$ is only taken by single policy among $\pi^*_{1},...\pi^*_k$.
% \footnote{As an intuitive example, for those MDPs with $A/2$ optimal actions at each state, it is possible that $\pi^*_i\neq \pi^*_j$ for arbitrary $1\leq i < j \leq k$ even if $k$ is $\text{Poly}(A,H)$, since the number of optimal deterministic policies $|\Pi^*| \geq (A/2)^H$ is at the exponential level.} 
We overcome this difficulty by proving the existence of ``well-covered'' policy in the theorem stated below:
% , in the proof of which we leverage the finite cardinality of state and action spaces.
% $\pi^*_i$ may not equal to $\pi^*_j$ when $i\neq j$, and therefore, it is hard no guarantee that there exists a policy $\pi^*\in\Pi^*$, which occurs in the policy sequence $\pi^*_1,...,\pi^*_k$ for $O(k)$ times. 
% As we will discuss in Sec. \ref{sec:tabular_RL_main_analysis} later, for the analysis of $\Regret(\algE)$, it is crucial to guarantee the existence of 
% Therefore, in order to show that the sub-optimality of $\piPVI_k$ can still gradually decay to zero with an appropriate rate, we need a stronger result to guarantee that there exists an optimal policy $\pi^*$ (maybe stochastic) ``well-covered'' by the sequence $\pi^*_1,...,\pi^*_k$, where the ``well-cover'' means that for each $(s_h,a_h)\in\cS\times\cA$ with $d^{\pi^*}(s_h,a_h) > 0$, we have $N_{k,h}(s_h,a_h)\sim \sum_{\tk=1}^k d^{\pi^*_\tk}(s_h,a_h) \sim O(k)$
% \footnote{Note that we may not guarantee that the policy obtained by a uniform mixture of $\pi_1^*,...\pi_k^*$ in Thm. \ref{thm:algO_regret_vs_algP_density} is ``well-covered'', because we may not infer the behavior of $\algO$ to guarantee the overlap between $\pi_1^*,...,\pi_k^*$. Therefore, we may not expect to obtain the constant regret by directly assigining such uniform policy as $\pi^*$ in the case (ii) in Thm. \ref{thm:clipping_trick} to obtain an upper bound and summing it over $k=1,2,...$ \red{do we need to mention this? to address the potential question about whether it is possible to consider the direct mixture of $\pi^*_1...,\pi_k^*$?}}
% Before stating the main theorem, we introduce two new notations. 
\begin{restatable}{theorem}{ThmExistWellCovered}[The existance of well-covered optimal policy]\label{thm:existence_of_well_covered_optpi}
    Given an arbitrary tabular MDP, and an arbitrary sequence of deterministic optimal policies $\pi^*_1,\pi^*_2,...\pi^*_\nk$ ($\pi^*_i$ may not equal to $\pi^*_j$ for arbitrary $1\leq i < j\leq \nk$ when there are multiple deterministic optimal policies), 
    % we use $I^*_\nk:=\{1,2,...,K\}$ to denote the index set. Then, there exists a subset $I\subset I^*_\nk$, and an optimal policy $\pi_{\text{cover}}:=\text{Uniform}(\{\pi^*_k:k\in I\})$ by uniformly mixing over the policies in the index set $I$ on the episode level, 
    there exists a (possibly stochastic) policy $\pi^*_{\text{cover}}$ 
    % which uniformly mixing a subset of policies among $\pi_1,...,\pi_\nk$, 
    such that $\forall h\in[H],\forall (s_h,a_h)\in\cS_h\times\cA_h$ with $d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0$:
    \begin{align*} 
        \sum_{\tk=1}^\nk d^{\pi^*_\tk}(s_h,a_h) \geq \frac{\nk}{2}\cdot \tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h),~ \text{with}~\tilde{d}^{\pi^*_{\text{cover}}}(\cdot,\cdot):= \max \left\{\frac{d^*_{h,\min}(\cdot,\cdot)}{(|\cZ_{h,\text{div}}|+1)H}, d^{\pi^*_{\text{cover}}}(\cdot,\cdot) \right\}.
    \end{align*}
    where $\cZ_{h,\text{div}}^* := \{(s_h,a_h)\in\cS_h\times\cA_h| \exists \pi^*, \tilde{\pi}^* \in \Pi^*,~ s.t.~ d^{\pi^*}(s_h) > 0,~ d^{\tilde{\pi}^*}(s_h) = 0\}$, and $d^*_{h,\min}(s_h,a_h):=\min_{\pi^*\in\Pi^*}d^{\pi^*}(s_h,a_h)$ subject to $d^{\pi^*}(s_h,a_h) > 0$.
\end{restatable}
Here we provide some explanation to the above result. According to the definition, $\cZ^*_{h,div}$ is the set including the state-action pairs which can be covered by some deterministic policies but is not reachable by some other deterministic policies, and therefore $|\cZ^*_{h,div}|\leq SA$ (or even $|\cZ^*_{h,div}| \ll SA$). Besides, $d^*_{h,\min}(s_h,a_h)$ denotes the minimal occupancy over all possible deterministic optimal policies which can hit $s_h,a_h$, and therefore, is no less than $d_{\min}$ defined in Thm.~\ref{thm:clipping_trick}. As a result, we know there exists a ``well-covered'' $\pi^*_{\text{cover}}$, since the accumulative density of its arbitrary reachable states can be lower bounded by $O(k)$. Then, following a similar discussion as the case $|\Pi^*|=1$,
% Then, combining with Thm. \ref{thm:algO_regret_vs_algP_density} and \ref{thm:clipping_trick}, 
we can finish the proof. We summarize our main result below.
% show the constant upper bound for $\Regret(\algE)$, which is stated in Thm.~\ref{thm:UB_Regret_PVI}, the main theorem of this section.
\begin{restatable}{theorem}{ThmUBPVI}\label{thm:UB_Regret_PVI}
    By running an Algorithm satisfying Condition~\ref{cond:requirement_on_algO} as $\algO$, running Alg~\ref{alg:PVI} as $\algE$ with a bonus term function $\textbf{Bonus}$ satisfying Condition~\ref{cond:bonus_term} and $\delta_k = 1/k^\alpha$, for some constant $\alpha > 1$, for arbitrary $K \geq 1$, the exploitation regret of $\algE$ can be upper bounded by:

    (i) When $|\Pi^*| = 1$ (unique optimal deterministic policy):
    % \begin{align*}
    %     \Regret_K(\algE) \leq &O\Big(\frac{\alpha H}{\alpha - 1} + \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} 
    %     \Big(\frac{\alpha(C_1+C_2)}{\Delta_{\min}}\log \frac{\alpha SAH(C_1+C_2)}{d^{\pi^*}(s_h,a_h) \Delta_{\min}} + \frac{\alpha B_1 H}{\Delta_{\min}}\log \frac{\alpha B_2 H}{d^{\pi^*}(s_h,a_h)\Delta_{\min}}\Big)\Big).
    % \end{align*}
    \begin{align*}
        \Regret_K(\algE) \leq &O\Big(\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} 
        \Big(\frac{C_1+C_2}{\Delta_{\min}}\log \frac{ SAH(C_1+C_2)}{d^{\pi^*}(s_h,a_h) \Delta_{\min}} + \frac{ B_1 H}{\Delta_{\min}}\log \frac{ B_2 H}{d^{\pi^*}(s_h,a_h)\Delta_{\min}}\Big)\Big).
    \end{align*}
    % \begin{align*}
    %     \Regret_K(\algE) \leq &\frac{3\alpha H}{\alpha - 1} + c_{\algE}\cdot \sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*}(s_h,a_h) > 0}} \Big(\frac{\alpha(C_1+C_2)}{\Delta_{\min}}\log \frac{\alpha SAH(C_1+C_2)}{d^{\pi^*}(s_h,a_h) \Delta_{\min}} \\
    %     & \qquad\qquad\qquad\qquad\qquad\qquad + \frac{\alpha B_1 H}{\Delta_{\min}}\log \frac{\alpha B_2 H}{d^{\pi^*}(s_h,a_h)\Delta_{\min}}\Big).
    % \end{align*}
    \indent (ii) When $|\Pi^*| > 1$ (non-unique optimal deterministic policies):
    \begin{align*}
        \Regret_K(\algE) \leq O\Big(\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0}} \Big(\frac{C_1+C_2}{\Delta_{\min}}\log \frac{ SAH(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)\Delta_{\min}} + \frac{ B_1 SAH}{d_{\min}\Delta_{\min}}\log \frac{ B_2 SAH}{d_{\min}\Delta_{\min}}\Big)\Big).
    \end{align*}
    % \begin{align*}
    %     \Regret_K(\algE) \leq &\frac{3\alpha H}{\alpha - 1} + c'_{\algE}\cdot\sum_{h=1}^H\sum_{\substack{s_h,a_h:\\d^{\pi^*_{\text{cover}}}(s_h,a_h) > 0}} \Big(\frac{\alpha(C_1+C_2)}{\Delta_{\min}}\log \frac{\alpha SAH(C_1+C_2)}{\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)\Delta_{\min}} \\
    %     & \qquad\qquad\qquad\qquad\qquad\qquad + \frac{\alpha B_1 SAH}{d_{\min}\Delta_{\min}}\log \frac{\alpha B_2 SAH}{d_{\min}\Delta_{\min}}\Big).
    % \end{align*}
    where 
    % $c_{\algE}$ and $c_{\algE}'$ are constants, 
    $\pi^*_{\text{cover}}$ and $\tilde{d}^{\pi^*_{\text{cover}}}(s_h,a_h)$ are introduced in Theorem \ref{thm:existence_of_well_covered_optpi}.
    % \red{TODO: take the minimum over $\log K$ if possible.}
\end{restatable}

% \blue{Because of the difficulty introduced by non-uniqueness of optimal policies, the regret bound depends on $\frac{1}{d_{\min}}$ instead of $\log \frac{1}{d_{\min}}$ under $|\Pi^*|=1$. 
% We conjecture it can be further improved and leave it to the future work (move blue sentence to conclusion?}.

\subsubsection{Interpretation of Results in Tabular RL}\label{sec:tabular_RL_Discussion}
% \subsubsection{Discussion}\label{sec:tabular_RL_Discussion}
% Finally, in Section \ref{sec:tabular_RL_Discussion} we conclude this section by investigating the additional dependence on $d^{\pi^*}$ in our regret bound.
% Besides, as a quick reminder, we will use $d^{\pi}(s_h,a_h):=\Pr(S_h=s_h,A_h=a_h|S_1=s_1,\pi)$ to denote the state action occupancy w.r.t. $\pi$.
Recall our objective in Sec.~\ref{sec:introduction} is to establish the benefits of leveraging the tiered structure by showing $\Regret_K(\algE)$ is constant. This contrasts the lower bound of online algorithms that continuously increases with the episode number $K$, which corresponds to the regret suffered by users in $\groupE$ without leveraging the tiered structure, while $\Regret_K(\algO)$ keeps (near-)optimal as before. In Appx.~\ref{appx:experiments}, we also provide some simulation results as a verification of our theoretical discovery.

One limitation of our results is that our bounds have additional dependence on $d^{\pi^*}$ (or even ${1}/{d^{\pi^*}}$) compared to most of the regret bounds in the online setting, although similar dependence on $\log d^{\pi^*}$ also appeared in a few recent works \citep[e.g., $\lambda_h^+$ in Thms. 8 and 9 of][]{papini2021reinforcement}. 
Besides, according to the lower and upper bound of online RL in gap-dependent settings \citep{simchowitz2019non},  $C_1+C_2$ in Cond.~\ref{cond:requirement_on_algO} have dependence on $O(\Delta_{\min}^{-1})$, which implies that in the regret bound in Thm.~\ref{thm:UB_Regret_PVI}, the dependence on $\Delta_{\min}$ would be $O(\Delta^{-2}_{\min})$.
For the former, in Appx.~\ref{appx:LB_Dep_Density}, we prove a lower bound, showing that $\log \frac{1}{d^{\pi^*}}$ is unavoidable when $\algO$ is allowed to behave adversarially without violating Cond.~\ref{cond:requirement_on_algO}; for the latter, we note that in the analysis of MAB setting (Sec.\ref{sec:analysis_for_MAB}), specifying the detailed behavior of $\algO$ can help tighten the bound.
% like what we did in Lemma \ref{lem:upper_bound_of_Nk_geq_k_div_A} for bandits.
% Although those the additional dependence on $d^{\pi^*}$ and the higher dependence on $\Delta_{\min}$ and other factors will decay the appearance of benefits, 
Therefore, we conjecture that our results can be improved by putting more constraints on the behavior of $\algO$, which we leave to future work.
% that we treat $\algO$ as a black-box algorithm. 
% satisfying Cond.~\ref{cond:requirement_on_algO} 
% without specifying its detailed behavior like what we did in Lemma \ref{lem:upper_bound_of_Nk_geq_k_div_A} for bandits.
% As a result, when $|\Pi^*|=1$, as we will .
% When $|\Pi^*|>1$, the situation becomes more complicated because we can only guarantee the existence of ``well-covered'' optimal policy (Theorem~ \ref{thm:existence_of_well_covered_optpi}), and have no idea about the overlap between that optimal policy and $\piPVI_k$ returned by PVI.
% As a result, in Thm.~\ref{thm:clipping_trick} we only guarantee an upper bound with a much smaller clipping threshold $\epsClip'$ compared to $\epsClip$, which leads to the additional $1/d_{\min}$ in the regret. 
% Besides, 
% We conjecture that similar to bandit setting (Sec. \ref{sec:analysis_for_MAB}), it is possible to get rid of the dependence on $d^{\pi^*}$ and improve the dependence on $\Delta_{\min}$ (and other factors like $S,A,H$) by considering an appropriate and concrete choice of $\algO$, which we leave to future work.


==> arxiv /notations.tex <==
\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\veps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}

% \renewcommand{\qedsymbol}{\hfill{\Large $\square$}}


\newcommand{\trans}{^{\top}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}

\newcommand{\bpi}{\bar{\pi}}
\newcommand{\btheta}{{\bm{\theta}}}
\newcommand{\pa}{{\pi_{\btheta+\Delta \btheta}}}
\newcommand{\pb}{{\pi_{\btheta}}}

\newcommand{\pta}[1]{{\pi_{\btheta+\Delta \btheta}^{#1}}}
\newcommand{\ptb}[1]{{\pi_{\boldsymbol{\theta}}^{#1}}}

\newcommand{\bL}{{\bm{L}}}

\newcommand{\dt}{{\Delta\btheta}}
\newcommand{\bt}{{\bm\theta}}
\newcommand{\dpt}{{\Delta\pb}}
\newcommand{\hV}{{\hat{V}}}
\newcommand{\hQ}{{\hat{Q}}}
\newcommand{\hB}{{\hat{B}}}
\newcommand{\hP}{{\hat{P}}}
\newcommand{\ph}{{h'}}
\newcommand{\pk}{{k'}}
\newcommand{\tk}{{\tilde{k}}}
\newcommand{\nk}{{k}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tQ}{\tilde{Q}}
\newcommand{\tR}{\tilde{R}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\hd}{\widehat{\text{DR}}}
\newcommand{\tpz}{\lim_{\dt\rightarrow \bm{0}}}
\newcommand{\gbt}{\nabla_{\btheta}}

\newcommand{\mB}{{\mathbb{B}}}
\newcommand{\mP}{{\mathbb{P}}}
\newcommand{\mR}{{\mathbb{R}}}
\newcommand{\mI}{{\mathbb{I}}}

\newcommand{\hmB}{{\hat{\mathbb{B}}}}
\newcommand{\hmP}{{\hat{\mathbb{P}}}}

\newcommand{\cov}{{\rm Cov}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\me}{{\mathbb{E}}}
\newcommand{\mv}{{\mathbb{V}}}
\newcommand{\trp}[1]{\Big(#1\Big)^2}

\newcommand{\si}{s_{\text{init}}}

\let\hat\widehat
\let\tilde\widetilde
% \let\check\widecheck
\def\given{{\,|\,}}
\def\biggiven{{\,\big|\,}}
\def\Biggiven{{\,\Big|\,}}
\def\bigggiven{{\,\bigg|\,}}
\def\Bigggiven{{\,\Bigg|\,}}
\def\ds{\displaystyle}
\newcommand\wtilde{\stackrel{\sim}{\smash{\mathcal{W}}\rule{0pt}{1.1ex}}}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{property}[theorem]{Property}
\newtheorem{claim}{Remark}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{objective}[theorem]{Objective}
\newtheorem{condition}[theorem]{Condition}
% \newtheorem{example}[theorem]{Example}
\newtheorem{assumption}{Assumption}
% \renewcommand*{\theassumption}{\Alph{assumption}}



% \def\##1\#{\begin{align}#1\end{align}}
% \def\$#1\${\begin{align*}#1\end{align*}}

\newcount\Comments  % 0 suppresses notes to selves in text
\Comments=1 % TODO: change to 0 for final version
\newcommand{\kibitz}[2]{\ifnum\Comments=1\textcolor{#1}{#2}\fi}
%\newcommand{\nan}[1]{\kibitz{blue}{[NJ: #1]}}


\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\gray}[1]{{\color{lightgray} #1}}

\newcommand{\pt}[2]{\frac{\partial #1}{\partial \theta_{#2}}}


\newcommand{\dti}[1]{{\epsilon_{#1}}}

\newcommand{\dpi}[2]{{\Delta\pi^{#1}_{\theta_{#2}}}}

\newcommand{\pai}[1]{{\pi_{\btheta+\dti{#1}\bm{e}_{#1}}}}

\newcommand{\tpzi}[1]{\lim_{\dti{#1}\rightarrow 0}}

\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\ptai}[2]{{\pi_{\btheta+\dti{#2}\bm{e}_{#2}}^{#1}}}

\newcommand{\diag}{{\rm Diag}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\algO}{\text{Alg}^\text{O}}
\newcommand{\algE}{\text{Alg}^\text{E}}
\newcommand{\alg}{\text{Alg}}
\newcommand{\envO}{\text{Env}^\text{O}}
\newcommand{\envE}{\text{Env}^\text{E}}
\newcommand{\env}{\text{Env}}
\newcommand{\piO}{{\pi}^\text{O}}
\newcommand{\piE}{{\pi}^\text{E}}
\newcommand{\piPVI}{{\pi}^\text{PVI}}
\newcommand{\groupO}{\text{G}^\text{O}}
\newcommand{\groupE}{\text{G}^\text{E}}
\newcommand{\tauO}{{\tau}^\text{O}}
\newcommand{\tauE}{{\tau}^\text{E}}

\newcommand{\surplus}{\mathbf{E}}
\newcommand{\Regret}{\text{Regret}}
\newcommand{\epsClip}{\epsilon_\text{Clip}}
\newcommand{\epsCliph}{\epsilon_\text{Clip,h}}
\newcommand{\Clip}{\text{Clip}}

\newcommand{\lf}{\lfloor}
\newcommand{\rf}{\rfloor}
\newcommand{\lc}{\lceil}
\newcommand{\rc}{\rceil}

\newcommand{\power}{\alpha}

\newcommand{\cEB}{\cE_{\textbf{Bonus}}}
\newcommand{\cECk}{\cE_{\textbf{Con},k}}
\newcommand{\cEBk}{\cE_{\textbf{Bonus},k}}
\newcommand{\cEOk}{\cE_{\algO,k}}


\newcommand{\cECnk}{\cE_{\textbf{Con},n,k}}
\newcommand{\cEBnk}{\cE_{\textbf{Bonus},n,k}}
\newcommand{\cEOnk}{\cE_{\algO,n,k}}

\newcommand{\btau}{\bar{\tau}}
\newcommand{\ttau}{\tilde{\tau}}
\newcommand{\mix}{\text{mix}}

% Definition of Events
\newcommand{\EmP}{E^{\text{prob}}}


\newcommand{\tOmega}{\tilde{\Omega}}
\newcommand{\tTheta}{\tilde{\Theta}}
\newcommand{\tO}{\tilde{O}}

\newcommand{\scalar}{\lambda}
\newcommand{\bscalar}{\bar{\lambda}}

\newcommand{\Gl}{G^{\text{lower}}}
\newcommand{\Gu}{G^{\text{upper}}}
